Free Algebra with Countable Basis

In this book I treat the structure of D-module which has countable basis. If we do not care for topology of D-module, then we consider Hamel basis. If norm is defined in D-module, then we consider Schauder basis. In case of Schauder basis, we consider vectors whose expansion in the basis converges normally.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 9780534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010)
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008)
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fihtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Center.Ring.Russian.tex <==
%auto-ignore
\input{Center.Ring.Eq}

\begin{definition}
\label{definition: center of ring}
Пусть $D$ - кольцо.\footnote{\citeBib{Serge Lang},
стр. 84.} Множество \symb{Z(D)}1{center of ring}
элементов $a\in D$ таких, что
\ShowEq{center of ring}
для всех $x\in D$,
называется
\AddIndex{центром кольца $D$}{center of ring}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: center of ring}
Центр $Z(D)$ кольца $D$ является подкольцом кольца $D$.
\end{theorem}
\begin{proof}
Непосредственно следует из определения \ref{definition: center of ring}.
\end{proof}

\begin{definition}
Пусть $D$ - кольцо с единицей $e$.\footnote{Определение
дано согласно
определению из \citeBib{Serge Lang},
стр. 84, 85.} Отображение
\[
l:Z\rightarrow D
\]
для которого $l(n)=ne$ будет гомоморфизмом колец, и его ядро является
идеалом $(n)$, порождённым целым числом $n\ge 0$.
Канонический инъективный гомоморфизм
\[
Z/nZ\rightarrow D
\]
является изоморфизмом между $Z/nZ$ и подкольцом в $D$.
Если $nZ$ - простой идеал, то у нас возникает два случая.
\begin{itemize}
\item $n=0$. $D$ содержит в качестве подкольца
кольцо, изоморфное $Z$ и часто отождествляемое
с $Z$. В этом случае мы говорим, что $D$ имеет
\AddIndex{характеристику $0$}{ring has characteristic 0}.
\item $n=p$ для некоторого простого числа $p$. $D$ имеет
\AddIndex{характеристику $p$}{ring has characteristic p}, и $D$
содержит изоморфный образ $F_p=Z/pZ$.
\end{itemize}
\qed
\end{definition}

\begin{theorem}
\label{theorem: integer subring of ring}
Пусть $D$ - кольцо характеристики $0$ и пусть $d\in D$.
Тогда любое целое число $n\in Z$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Утверждение теоремы доказывается по индукции.
При $n=0$ и $n=1$ утверждение очевидно.
Допустим утверждение справедливо при $n=k$.
Из цепочки равенств
\[
(k+1)d=kd+d=dk+d=d(k+1)
\]
следует очевидность утверждения при $n=k+1$.
\end{proof}

\begin{theorem}
\label{theorem: integer subring of center}
Пусть $D$ - кольцо характеристики $0$.
Тогда кольцо целых чисел $Z$ является подкольцом центра $Z(D)$ кольца $D$.
\end{theorem}
\begin{proof}
Следствие теоремы \ref{theorem: integer subring of ring}.
\end{proof}


==> Convention.Russian.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Соглашения}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\begin{convention}
Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{Calculus.Paper,BVector}
\ifx\Semafor\ValueOn
\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $s$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\begin{convention}
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
При этом подразумевается, что отображение мультипликативно над
максимально возможным полем. В частности, линейное отображение
тела $D$ мультипликативно над центром $Z(D)$. Это не противоречит
определению линейного отображения поля, так как для поля $F$ справедливо
$Z(F)=F$.
Если поле $F$ отлично
от максимально возможного, то я это явно указываю в тексте.
\qed
\end{convention}
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\begin{convention}
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
Запись \Ds линейно зависимые векторы можно прочесть
как D\Hyph star\Hyph линейно зависимые векторы либо
как векторы, линейно зависимые слева.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,BVector,CACAA.07.195}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - свободная конечно
мерная алгебра.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
Однако в алгебре не принято использовать векторные обозначения.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,CACAA.07.195}
\ifx\Semafor\ValueOn
\begin{convention}
Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\qed
\end{convention}
\fi

\ePrints{1104.5197,1105.4307}
\ifx\Semafor\ValueOn
\begin{convention}
Хотя алгебра является свободным модулем над некоторым
кольцом, мы не пользуемся векторными обозначениями
при записи элементов алгебры. В тех случаях, когда я рассматриваю
матрицу координат элемента алгебры, я буду пользоваться векторными
обозначениями для записи соответствующего элемента.
Чтобы не возникала неоднозначность при записи сопряжения,
я буду обозначать $a^*$ элемент, сопряжённый элементу $a$.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072,1111.6035,1102.5168}
\ifx\Semafor\ValueOn
\begin{convention}
В \citeBib{Cohn: Universal Algebra}
произвольная операция алгебры обозначена буквой $\omega$,
и $\Omega$ - множество операций некоторой универсальной алгебры.
Соответственно, универсальная алгебра с множеством операций
$\Omega$ обозначается $\Omega$\Hyph алгебра.
Аналогичные обозначения мы видим в
\citeBib{Burris Sankappanavar} с той небольшой разницей,
что операция в алгебре обозначена буквой $f$
и $\mathcal F$ - множество операций.
Я выбрал первый вариант обозначений, так как в этом случае
легче видно, где я использую операцию.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072}
\ifx\Semafor\ValueOn
\begin{convention}
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
\ePrints{8443-0072}
\ifx\Semafor\ValueOn
Символом
\else
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом
\fi
$\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\VX A,\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.
\qed
\end{convention}

\begin{convention}
Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\qed
\end{convention}
\fi

\ePrints{8443-0072,1111.6035,0906.0135,NewAffine,1102.5168}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - $\Omega_1$\Hyph алгебра.
Пусть $B$ - $\Omega_2$\Hyph алгебра.
Запись
\ShowEq{A->*B}
означает, что определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
\qed
\end{convention}
\fi

\ePrints{0702.561,0707.2246,0803.2620}
\ifx\Semafor\ValueOn
\begin{convention}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
\qed
\end{convention}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\begin{remark}
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\qed
\end{remark}
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\begin{convention}
Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\qed
\end{convention}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Пусть $\VX X$ - базис башни представлений $(\Vector A,\Vector f)$.
%Мы будем называть $\Omega_n$\Hyph слово
%$w_n(\Vector f,\VX X,x_n)$ координатами $x_n\in A_n$
%относительно базиса $\VX X$.
%\fi

\ePrints{1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
Для данной $D$\Hyph алгебры $A$
левый сдвиг
\ShowEq{left shift, D algebra}
определён равенством
\ShowEq{left shift 1, D algebra}
и правый сдвиг
\ShowEq{right shift, D algebra}
определён равенством
\ShowEq{right shift 1, D algebra}
\qed
\end{convention}
\fi

\ifx\PrintPaper\undefined
Без сомнения, у читателя могут быть вопросы,
замечания, возражения. Я буду признателен любому отзыву.
\fi



==> Hamel.Basis.Russian.tex <==
%auto-ignore
\input{Hamel.Basis.Eq}
\ifx\PrintBook\Defined
\chapter{Базис Гамеля}
\fi

\section{Модуль}
\label{Section: Module}

\begin{theorem}
\label{theorem: effective representation of the ring}
Пусть кольцо $D$ имеет единицу $e$.
Представление\footnote{Этот подраздел
написан на основе раздела
\xRef{8433-5163}{Section: Module}.}
\ShowEq{representation of the ring}
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation of ring}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
\end{theorem}
\begin{proof}
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{sum of transformations of Abelian group}
Поэтому, рассматривая представление кольца $D$ в
абелевой группе $A$, мы полагаем
\ShowEq{sum of transformations of Abelian group, 1}
Произведение преобразований представления определено
согласно правилу
\ShowEq{product of transformations of representation}

Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенства
\EqRef{representation of ring, 1}
следует, что $a-b$ порождает нулевое преобразование
\ShowEq{representation of ring, 2}
Элемент $e+a-b$ порождает тождественное преобразование.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
\end{proof}

\begin{definition}
\label{definition: module over ring}
Пусть $D$ - коммутативное кольцо.
Эффективное представление кольца $D$
в абелевой группе $A$ называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: definition of module}
Элементы $D$\Hyph модуля $A$ удовлетворяют
соотношениям:
\begin{itemize}
\item 
\AddIndex{закону ассоциативности}{associative law, D module}
\ShowEq{associative law, D module}
\item 
\AddIndex{закону дистрибутивности}{distributive law, D module}
\ShowEq{distributive law, D module}
\item 
\AddIndex{закону унитарности}{unitarity law, D module}
\ShowEq{unitarity law, D module}
\end{itemize}
для любых
\ShowEq{definition of module}
\end{theorem}
\begin{proof}
Равенство \EqRef{distributive law, D module, 1} следует
из утверждения, что преобразование $a$ является эндоморфизмом абелевой группы.
Равенство \EqRef{distributive law, D module, 2} следует
из утверждения, что представление является гомоморфизмом аддитивной группы
кольца $D$.
Равенства \EqRef{associative law, D module} и
\EqRef{unitarity law, D module} следуют
из утверждения, что представление кольца $D$ является
представлением мультипликативной группы кольца $D$.
\end{proof}

Векторы
\ShowEq{Vector A subs row, 1}
$D$\Hyph модуля $A$ \AddIndex{$D$\Hyph линейно независимы}
{D linearly independent, module}\footnote{Я следую
определению в \citeBib{Serge Lang}, с. 100.},
если $c=0$ следует из уравнения
\ShowEq{rcd linearly independent}
В противном случае, векторы \ShowEq{Vector A subs row, 1}
\AddIndex{$D$\Hyph линейно зависимы}{D linearly dependent, module}.

\begin{definition}
\label{definition: free module over ring}
Множество векторов
\ShowEq{basis, module}
- \AddIndex{$D$ базис модуля}{D basis, module},
если векторы $\Veb$ $D$\Hyph линейно независимы и добавление
любого вектора к этой системе
делает эту систему $D$\Hyph линейно зависимой.
$A$ - \AddIndex{свободный модуль над кольцом}{free module over ring} $D$,
если $A$ имеет базис
над кольцом $D$.\footnote{Я следую
определению в \citeBib{Serge Lang}, с. 103.}
\qed
\end{definition}

Следующее определение является следствием определений
\ref{definition: module over ring}
и \xRef{8443-0072}{definition: morphism of representations of F algebra}.

\begin{definition}
\label{definition: linear map from A1 to A2, module}
Пусть $A_1$ и
$A_2$ - модули над кольцом $D$.
Морфизм
\ShowEq{linear map from A1 to A2}
представления кольца $D$ в абелевой группе $A_1$
в представление кольца $D$ в абелевой группе $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear map from A1 to A2}
Линейное отображение
\ShowEq{linear map from A1 to A2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
удовлетворяет равенствам\footnote{В некоторых книгах
(например, \citeBib{Serge Lang}, с. 94)
теорема \ref{theorem: linear map from A1 to A2}
рассматривается как определение.}
\ShowEq{linear map from A1 to A2, 1}
\end{theorem}
\begin{proof}
Из определения
\ref{definition: linear map from A1 to A2, module}
и теоремы
\xRef{8443-0072}{theorem: morphism of representations of algebra, reduce}
следует, что
отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\EqRef{linear map from A1 to A2, 1 1}).
Равенство
\EqRef{linear map from A1 to A2, 1 2}
следует из равенства
\xEqRef{8443-0072}{morphism of representations of F algebra}.
\end{proof}

\begin{theorem}
Пусть $A_1$ и
$A_2$ - модули над кольцом $D$.
Множество $\LDA$
является абелевой группой
относительно закона композиции
\ShowEq{sum of linear maps}
\ShowEq{sum of linear maps, definition}
который называется
\AddIndex{суммой линейных отображений}{sum of linear maps}.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: linear map from A1 to A2, module}
\ShowEq{sum of linear maps 1, module}
Слудовательно, отображение,
определённое равенством \EqRef{sum of linear maps, definition},
является линейным отображением $D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$.
Коммутативность и ассоциативность сложения
следует из равенств
\ShowEq{sum of linear maps 2, module}

Определим отображение
\ShowEq{0 circ x}
Очевидно,
\ShowEq{0 in L}
Из равенства
\ShowEq{0+f circ}
следует
\ShowEq{0+f}

Определим отображение
\ShowEq{-f circ x}
Очевидно,
\ShowEq{-f in L}
Из равенства
\ShowEq{-f+f circ}
следует
\ShowEq{-f+f}

Следовательно, множество $\LDA$
является абелевой группой.
\end{proof}

\begin{theorem}
Пусть $A_1$ и
$A_2$ - модули над кольцом $D$.
Представление кольца $D$ в абелевой группе $\LDA$,
определённое равенством
\ShowEq{product of map over scalar}
\ShowEq{product of map over scalar, definition}
называется
\AddIndex{произведением отображения на скаляр}
{product of map over scalar}.
Это представление порождает структуру $D$\Hyph модуля
в абелевой группе $\LDA$.
\end{theorem}
\begin{sloppypar}
\begin{proof}
Из равенств
\ShowEq{f->df 1}
следует, что отображение
\ShowEq{f->df}
является преобразованием множества $\LDA$.
Из равенства
\ShowEq{f->df 2}
следует, что отображение
\EqRef{f->df}
является гомоморфизмом абелевой группы $\LDA$.
Согласно определению
\xRef{8433-5163}{definition: module over ring},
абелевая группа $\LDA$ является $D$\Hyph модулем.
\end{proof}
\end{sloppypar}

\begin{definition}
\label{definition: conjugated D module}
Пусть $A$ - $D$\Hyph  модуль.
$D$\Hyph  модуль
\ShowEq{conjugated D module}
называется
\AddIndex{сопряжённым $D$\Hyph модулем}{conjugated D module}.
\qed
\end{definition}

Согласно определению
\ref{definition: conjugated D module},
элементы сопряжённого $D$\Hyph модуля
являются $D$\Hyph линейными отображениями
\ShowEq{conjugated D module 1}
$D$\Hyph линейное отображение
\EqRef{conjugated D module 1}
называется
\AddIndex{линейным функционалом на $D$\Hyph модуле}
{linear functional, D module}
$A$ или просто
\AddIndex{$D$\Hyph линейным функционалом}{D linear functional}.

\begin{theorem}
Пусть
\ShowEq{basis of module A}
- базис $D$\Hyph модуля $A$.
Пусть $A'$ - $D$\Hyph модуль, сопряжённый $D$\Hyph модулю $A$.
Множество векторов
\ShowEq{basis of module A'}
такой, что
\ShowEq{basis of module A A'}
является базисом $D$\Hyph модуля $A'$.
\end{theorem}
\begin{proof}
Из равенства
\EqRef{basis of module A A'}
следует, что
\ShowEq{basis of module A A' 1}
Пусть
\ShowEq{f:A->D}
линейное отображение. Тогда
\ShowEq{basis of module A A' 2}
где
\ShowEq{fi}
Из равенств
\EqRef{basis of module A A' 1},
\EqRef{basis of module A A' 2}
следует, что
\ShowEq{basis of module A A' 3}
Согласно определениям
\EqRef{sum of linear maps, definition},
\EqRef{product of map over scalar, definition}
\ShowEq{basis of module A' 1}
Следовательно, множество
\ShowEq{basis of module A'}
является базисом $D$\Hyph модуля $A'$.
\end{proof}

\begin{corollary}
\label{corollary: basis of module A'}
Пусть
\ShowEq{basis of module A}
- базис $D$\Hyph модуля $A$.
Тогда
\ShowEq{ai=ei a}
\qed
\end{corollary}

Базис
\ShowEq{basis of module A'}
называется
\AddIndex{базисом, двойственным базису}{dual basis}
\ShowEq{basis of module A}.

\begin{theorem}
\label{theorem: basis of module A1 A2}
Пусть
\ShowEq{basis of module A1}
- базис $D$\Hyph модуля $A_1$.
Пусть
\ShowEq{basis of module A2}
- базис $D$\Hyph модуля $A_2$.
Множество векторов
\ShowEq{basis of module A1 A2}
определённых равенством
\ShowEq{basis L(A1,A2)}
является базисом $D$\Hyph модуля $\LDA$.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{f:A1->A2}
отображение $D$\Hyph модуля $A_1$ с базисом $\Basis e_1$
в $D$\Hyph модуль $A_2$ с базисом $\Basis e_2$.
Пусть
\ShowEq{a in A1}
Согласно следствию
\ref{corollary: basis of module A'}
\ShowEq{fa=,1}
Так как
\ShowEq{fa=,2}
то из равенства
\EqRef{fa=,1}
следует
\ShowEq{fa=,3}
Из равенств
\EqRef{basis L(A1,A2)},
\EqRef{fa=,3}
следует
\ShowEq{fa=,4}
Следовательно,
\ShowEq{fa=,5}
Так как отображения
\EqRef{basis L(A1,A2)}
линейно независимы,
то множество этих отображений является базисом.
\end{proof}

\begin{definition}
\label{definition: polylinear map of modules}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Мы будем называть отображение
\ShowEq{polylinear map of algebras}
\AddIndex{полилинейным отображением}{polylinear map} модулей
$A_1$, ..., $A_n$
в модуль $S$,
если
\ShowEq{polylinear map of algebras, 1}
\qed
\end{definition}

\section{Алгебра над кольцом}
\label{section: Algebra over Ring}

\begin{definition}
\label{definition: algebra over ring}
Пусть $D$ - коммутативное кольцо.\footnote{Этот
раздел написан на основе раздела
\xRef{8433-5163}{section: Algebra over Ring}.}
$A$ - \AddIndex{алгебра над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгебра}{D algebra},
если $A$ - $D$\Hyph модуль и в $A$
определена операция произведения\footnote{Я следую определению, приведенному в
\citeBib{Richard D. Schafer}, с. 1,
\citeBib{0105.155}, с. 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.}
\ShowEq{product in algebra, definition 1}
где $f$ билинейное отображение
\ShowEq{product in algebra, definition 2}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
\qed
\end{definition}

Согласно построениям, выполненным в разделах
\xRef{8443-0072}{subsection: Free Algebra over Ring},
\xRef{8443-0072}{subsection: n algebra},
диаграмма представлений $D$\Hyph алгебры имеет вид
\ShowEq{diagram of representations of D algebra}
На диаграмме представлений
\EqRef{diagram of representations of D algebra},
$D$ - кольцо, $A$ - абелевая группа.
Мы сперва рассматриваем вертикальное представление,
а затем горизонтальные.

\begin{theorem}
Произведение в алгебре $A$ дистрибутивно по отношению к сложению.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{product distributive in algebra}
\end{proof}

\begin{definition}
\label{definition: linear map from A1 to A2, algebra}
Пусть $A_1$ и
$A_2$ - алгебры над кольцом $D$.
Линейное отображение
\ShowEq{linear map from A1 to A2}
$D$\hyph модуля $A_1$
в $D$\hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Обозначим
\ShowEq{set linear maps, algebra}
множество линейных отображений
алгебры
$A_1$
в алгебру
$A_2$.
\qed
\end{definition}

\begin{theorem}
Если на $D$\Hyph модуле $\LDa$
определить произведение
\ShowEq{(fg)a=f(ga)}
то $\LDa$ является $D$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Из равенств
\ShowEq{fg 1}
следует, что отображение
\ShowEq{fg}
билинейно.
Согласно определению
\ref{definition: algebra over ring},
$D$\Hyph модуль $\LDa$ является $D$\Hyph алгеброй.
\end{proof}

Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данным в \citeBib{Richard D. Schafer}, с. 13.

\begin{definition}
\label{definition: commutator of algebra}
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
\qed
\end{definition}

\begin{definition}
\label{definition: associator of algebra}
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
\qed
\end{definition}

\begin{definition}
\label{definition: nucleus of algebra}
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это множество\footnote{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13}
\ShowEq{nucleus of algebra}
\qed
\end{definition}

\begin{definition}
\label{definition: center of algebra}
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это множество\footnote{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 14}
\ShowEq{center of algebra}
\qed
\end{definition}

\begin{theorem}
Пусть $\Basis e$ - базис свободной конечномерной алгебры $A$ над кольцом $D$.
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\DrawEq{product ab in algebra}{1}
где
\ShowEq{structural constants of algebra}
- \AddIndex{структурные константы алгебры}{structural constants}
$A$ над кольцом $D$.
Произведение базисных векторов в алгебре $A$ определено согласно правилу
\DrawEq{product of basis vectors}{algebra}
\end{theorem}
\begin{proof}
Равенство
\eqRef{product of basis vectors}{algebra}
является следствием утверждения, что $\Basis e$
является базисом алгебры $A$.
Так как произведение в алгебре является билинейным отображением,
то произведение $a$ и $b$ можно записать в виде
\DrawEq{product ab in algebra, 1}{1}
Из равенств
\eqRef{product of basis vectors}{algebra},
\eqRef{product ab in algebra, 1}{1},
следует
\DrawEq{product ab in algebra, 2}{1}
Так как $\Basis e$ является базисом алгебры $A$, то равенство
\eqRef{product ab in algebra}{1}
следует из равенства
\eqRef{product ab in algebra, 2}{1}.
\end{proof}

\section{\texorpdfstring{$D$}{D}\hyph алгебра с базисом Гамеля}

Если $D$\Hyph модуль $A$ имеет счётный базис $\Basis e$,
то бесконечная сумма в $D$\Hyph модуле $A$,
вообще говоря, не определена.
Если в $D$\Hyph модуле $A$ не определенно понятие
непрерывности, мы будем опираться на следующее определение
(\citeBib{0 521 59180 5}, с. 223).

\begin{definition}
\label{definition: module, Hamel basis}
Пусть $D$\Hyph модуль $A$ имеет счётный базис
\ShowEq{Hamel basis}
Если любой элемент
$D$\Hyph модуля $A$ имеет конечное разложение относительно базиса $\Basis e$,
а именно, в равенстве
\ShowEq{a=ai ei}
множество значений $a^{\gi i}\in D$, отличных от $0$, конечно,
то базис $\Basis e$ называется
\AddIndex{базисом Гамеля}{Hamel basis}.
Последовательность скаляров 
\ShowEq{Hamel basis, coordinates}
называется
\AddIndex{координатами вектора
\ShowEq{a=ai ei}
относительно базиса Гамеля}
{coordinates of vector, Hamel basis}
$\Basis e$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear map, module, Hamel basis}
Пусть
\ShowEq{f:A1->A2}
отображение $D$\Hyph модуля $A_1$ с базисом Гамеля $\Basis e_1$
в $D$\Hyph модуль $A_2$ с базисом Гамеля $\Basis e_2$.
Пусть $f^{\gi i}_{\gi j}$ - координаты отображения $f$
относительно базисов $\Basis e_1$ и $\Basis e_2$.
Тогда для любого $\gi j$,
множество значений $f^{\gi i}_{\gi j}$, отличных от $0$, конечно.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из равенства
\ShowEq{f:A1->A2, 1}
\end{proof}

\begin{theorem}
Пусть
\ShowEq{f:A1->A2}
линейное отображение $D$\Hyph модуля $A_1$ с базисом Гамеля $\Basis e_1$
в $D$\Hyph модуль $A_2$ с базисом Гамеля $\Basis e_2$.
Тогда для любого $a_1\in A_1$, образ
\DrawEq{f:A1->A2, 2}{Hamel}
определён корректно.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{a1 in A1}
Согласно определению
\ref{definition: module, Hamel basis},
множество значений $a^{\gi j}$, отличных от $0$, конечно.
Пусть $f^{\gi i}_{\gi j}$ - координаты отображения $f$
относительно базисов $\Basis e_1$ и $\Basis e_2$.
Согласно теореме
\ref{theorem: linear map, module, Hamel basis},
для любого $\gi j$,
множество значений $f^{\gi i}_{\gi j}$, отличных от $0$, конечно.
Объединение конечного множества конечных множеств является
конечным множеством.
Следовательно,
множество значений $a_1^{\gi j}f^{\gi i}_{\gi j}$, отличных от $0$, конечно.
Согласно определению
\ref{definition: module, Hamel basis},
выражение
\eqRef{f:A1->A2, 2}{Hamel}
является разложением элемента $a_2$ относительно базиса Гамеля $\Basis e_2$.
\end{proof}

\begin{convention}
%\label{convention: }
Пусть $\Basis e$ - базис Гамеля свободной $D$\Hyph алгебры $A$.
Произведение базисных векторов в $D$\Hyph алгебре $A$
определено согласно правилу
\DrawEq{product of basis vectors}{Hamel basis}
где
\ShowEq{structural constants of algebra}
- \AddIndex{структурные константы}{structural constants}
$D$\Hyph алгебры $A$.
Так как произведение векторов базиса $\Basis e$
$D$\Hyph алгебры $A$ является вектором $D$\Hyph алгебры $A$, то
мы требуем, что
для любых $\gi i$, $\gi j$,
множество значений $C^{\gi k}_{\gi{ij}}$, отличных от $0$,
конечно.
\qed
\end{convention}

\begin{theorem}
Пусть $\Basis e$ - базис Гамеля свободной $D$\Hyph алгебры $A$.
Тогда для любых
\ShowEq{a b in basis of algebra}
произведение, определённое согласно правилу
\DrawEq{product ab in algebra}{Hamel basis}
определено корректно.
\end{theorem}
\begin{proof}
Так как произведение в алгебре является билинейным отображением,
то произведение $a$ и $b$ можно записать в виде
\DrawEq{product ab in algebra, 1}{Hamel basis}
Из равенств
\eqRef{product of basis vectors}{Hamel basis},
\eqRef{product ab in algebra, 1}{Hamel basis},
следует
\DrawEq{product ab in algebra, 2}{Hamel basis}
Так как $\Basis e$ является базисом алгебры $A$, то равенство
\eqRef{product ab in algebra}{Hamel basis}
следует из равенства
\eqRef{product ab in algebra, 2}{Hamel basis}.

Поскольку базис $\Basis e$ - базис Гамеля, то
\begin{itemize}
\item множество значений $a^{\gi i}$, отличных от $0$, конечно;
\item множество значений $b^{\gi j}$, отличных от $0$, конечно.
\end{itemize}
Следовательно, множество произведений $a^{\gi i}b^{\gi j}$,
отличных от $0$, конечно.
Для любых $\gi i$, $\gi j$,
множество значений $C^{\gi k}_{\gi{ij}}$, отличных от $0$, конечно.
Следовательно, произведение определено равенством
\eqRef{product ab in algebra}{Hamel basis}
корректно.
\end{proof}

\begin{theorem}
\label{theorem: standard component of tensor, algebra, Hamel basis}
Пусть $A_1$, ..., $A_n$ -
свободные алгебры над  коммутативным кольцом $D$.
Пусть $\Basis e_i$ - базис Гамеля $D$\Hyph алгебры $A_i$.
Тогда множество векторов
\ShowEq{tensor, algebra, Hamel basis}
является базисом Гамеля тензорного произведения
\ShowEq{tensor, algebra, Hamel basis, 1}
\end{theorem}
\begin{proof}
Для доказательства теоремы мы должны рассмотреть диаграмму
\xEqRef{8433-5163}{diagram top, algebra, tensor product},
которой мы пользовались для доказательства теоремы
\xRef{8433-5163}{theorem: tensor product of algebras is module}
\ShowEq{standard component of tensor, algebra, Hamel basis, diagram}
Пусть $M_1$ - модуль над кольцом $D$, порождённый
произведением $\Times$
$D$\Hyph алгебр $A_1$, ..., $A_n$.
\begin{itemize}
\item
Пусть вектор $b\in M_1$ имеет конечное разложение
относительно базиса $\Times$
\ShowEq{b in M_1, Hamel basis}
где $I_1$ - конечное множество.
Пусть вектор $c\in M_1$ имеет конечное разложение
относительно базиса $\Times$
\ShowEq{c in M_1, Hamel basis}
где $I_2$ - конечное множество.
Множество
\ShowEq{I=I1+I2}
является конечным множеством.
Положим
\ShowEq{b I2, c I1}
Тогда
\ShowEq{b+c in M_1, Hamel basis}
где $I$ - конечное множество.
Аналогично, для $d\in D$
\ShowEq{db in M_1, Hamel basis}
где $I_1$ - конечное множество.
Следовательно, мы доказали следующее утверждение.\footnote{Множество
$\Times$ не может быть базисом Гамеля, так как
это множество не счётно.}
\begin{lemma}
\label{lemma: M is submodule}
Множество $M$ векторов модуля $M_1$, имеющих конечное разложение
относительно базиса $\Times$, является подмодулем модуля $M_1$.
\end{lemma}
\end{itemize}
Инъекция
\ShowEq{map i, algebra, tensor product, 1}
определена по правилу
\ShowEq{map i, algebra, Hamel basis, tensor product}
Пусть $N\subset M$ - подмодуль, порождённый элементами вида
\ShowEq{kernel, algebra, Hamel basis, tensor product}
где $d_i\in A_i$, $c_i\in A_i$, $a\in D$.
Пусть
\[
j:M\rightarrow M/N
\]
каноническое отображение на фактормодуль.
Поскольку элементы \EqRef{kernel 1, algebra, Hamel basis, tensor product}
и \EqRef{kernel 2, algebra, Hamel basis, tensor product}
принадлежат ядру линейного отображения $j$,
то из равенства
\EqRef{map i, algebra, Hamel basis, tensor product}
следует
\ShowEq{f, algebra, Hamel basis, tensor product}
Из равенств \EqRef{f 1, algebra, Hamel basis, tensor product}
и \EqRef{f 2, algebra, Hamel basis, tensor product}
следует, что отображение $f$ полилинейно над кольцом $D$.

Модуль $M/N$ является тензорным произведением $A_1\otimes...\otimes A_n$,
отображение $j$ имеет вид
\ShowEq{map j, Hamel basis}
и множество
тензоров вида
\ShowEq{tensor, algebra, Hamel basis}
является счётным базисом модуля $M/N$.
Согласно лемме
\ref{lemma: M is submodule},
произвольный вектор
\ShowEq{b in M, Hamel basis, 0}
имеет представление
\ShowEq{b in M, Hamel basis}
где $I$ - конечное множество.
Согласно определению
\EqRef{map j, Hamel basis}
отображения $j$
\ShowEq{j(b), Hamel basis}
где $I$ - конечное множество.
Так как $\Basis e_k$ - базис Гамеля $D$\Hyph алгебры $A_k$,
то для любого набора индексов $k\cdot i$, в равенстве
\ShowEq{aki, Hamel basis}
множество значений
\ShowEq{aki 1, Hamel basis}
отличных от $0$, конечно.
Следовательно, равенство
\EqRef{j(b), Hamel basis}
имеет вид
\ShowEq{j(b), 1, Hamel basis}
где множество значений
\ShowEq{j(b), 2, Hamel basis}
отличных от $0$, конечно.
\end{proof}

\begin{corollary}
\label{corollary: tensor product, Hamel basis}
Пусть $A_1$, ..., $A_n$ -
свободные алгебры над  коммутативным кольцом $D$.
Пусть $\Basis e_i$ - базис Гамеля $D$\Hyph алгебры $A_i$.
Тогда произвольный тензор $a\in A_1\otimes...\otimes A_n$
имеет конечное множество стандартных компонент,
отличных от $0$.
\qed
\end{corollary}

\begin{theorem}
Пусть $A_1$ - алгебра
над кольцом $D$.
Пусть $A_2$ - свободная ассоциативная алгебра
над кольцом $D$ с базисом Гамеля $\Basis e$.
Отображение
\ShowEq{standard representation of map A1 A2, 1, Hamel basis}
порождённое отображением $f\in\LDA$
посредством тензора $a\in\ATwo$, имеет стандартное представление
\ShowEq{standard representation of map A1 A2, 2, Hamel basis}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: standard component of tensor, algebra, Hamel basis},
стандартное представление тензора $a$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, Hamel basis}
Равенство
\EqRef{standard representation of map A1 A2, 2, Hamel basis}
следует из равенств
\EqRef{standard representation of map A1 A2, 1, Hamel basis},
\EqRef{standard representation of map A1 A2, 3, Hamel basis}.
\end{proof}


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-rcd форма
   {$1$-\rcd форма}%
   {1-rcd form, vector spaces}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%668%A%A CRcirc- базис модуля
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Index%667%A%A CRcirc- линейно ависимое множество векторов
   {$A\CRcirc$\Hyph линейно зависимое множество векторов}%
   {CRcirc linearly dependent, Astar module over algebra}%
\Index%666%A%A CRcirc- линейно независимое множество векторов
   {$A\CRcirc$\Hyph линейно независимое множество векторов}%
   {CRcirc linearly independent, Astar module over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%693%A%A линейное отображение модулей
   {$A$\Hyph линейное отображение модулей}%
   {A linear map of modules}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%680%A%Acr линейное отображение модулей
   {\Acr линейное отображение модулей}%
   {Acr linear map of modules}%
\Index%764%A%ACRcirc линейная комбинация
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%789%A%Astar антилинейное отображение алгебры с сопряжением
   {$A\star$\Hyph антилинейное отображение алгебры с сопряжением}%
   {antilinear mapping of algebra with conjugation}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%665%A%Astar- произведение вектора на скаляр
   {$A\star$\Hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, Astar module}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%13%C%crd производная Гато отображения \Vector f D-векторного пространства \Vector V в D-векторное пространство \Vector W
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%659%D%D- базис модуля
   {$D$\Hyph базис модуля}%
   {D basis, module}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%658%D%D линейно зависимые векторы D модуля
   {$D$\Hyph линейно зависимые векторы $D$\Hyph модуля}%
   {D linearly dependent, module}%
\Index%657%D%D линейно независимые векторы D модуля
   {$D$\Hyph линейно независимые векторы $D$\Hyph модуля}%
   {D linearly independent, module}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%20%D%Drc  линейно зависимые векторные поля
   {\Drc  линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%19%D%drc векторное пространство r строк
   {\drc векторное пространство \subs строк}%
   {subs rows drc vector space}%
\Index%33%D%Drc линейно независимые векторные поля
   {\Drc линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%70%D%drc представление группы
   {\drc представление группы}%
   {drc linear representation of group}%
\Index%38%D%drc производная Гато отображения \Vector f D- векторного пространства \Vector V в D- векторное пространство \Vector W
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Index%779%D%Dstar антилинейное отображение кольца с сопряжением
   {$D\star$\Hyph антилинейное отображение кольца с сопряжением}%
   {antilinear mapping of ring with conjugation}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%734%D%Dstar аффинное пространство
   {$D\star$\Hyph аффинное пространство}%
   {Dstar affine space}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%42%D%Dstar компонента координат вектора \Vector r
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Index%769%D%Dstar линейный гомоморфизм
   {$D\star$\Hyph линейный гомоморфизм}%
   {Dstar linear homomorphism}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%156%D%Dstar-модуль
   {$D\star$\Hyph модуль}%
   {Dstar-module}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index%32%D%rcd линейная оболочка в векторном пространстве
   {\rcd линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%726%N%n алгебра над кольцом
   {$n$\Hyph алгебра над кольцом}%
   {n algebra over ring}%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%49%R%drc базис, дуальный rcd базису в векторном пространстве
   {\drc базис, дуальный \rcd базису в векторном пространстве}%
   {basis dual to basis, rcd vector space}%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%677%R%RCcirc A- базис модуля
   {$\RCcirc A$\Hyph базис модуля}%
   {RCcirc A basis, module over algebra}%
\Index%676%R%RCcirc A- линейно ависимое множество векторов
   {$\RCcirc A$\Hyph линейно зависимое множество векторов}%
   {RCcirc linearly dependent, starA module over algebra}%
\Index%675%R%RCcirc A- линейно независимое множество векторов
   {$\RCcirc A$\Hyph линейно независимое множество векторов}%
   {RCcirc linearly independent, starA module over algebra}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%765%R%RCcircA линейная комбинация
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination}%
\Index%22%R%rcd автоморфизм векторного пространства
   {\rcd автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%758%R%rcd аффинное преобразование
   {\rcd аффинное преобразование}%
   {rcd affine transformation}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%29%R%rcd векторное пространство c строк
   {\rcd векторное пространство \sups строк}%
   {sups rows rcd vector space}%
\Index%31%R%rcd изоморфизм векторных пространств
   {\rcd изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%37%R%rcd линейным Tstar- представление группы
   {\rcd линейным \Ts представление группы}%
   {rcd linear Tstar representation of group}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index%77%S%Dstar- произведением rcd линейного отображения A на скаляр
   {$D\star$\Hyph произведением \rcd линейного отображения $A$ на скаляр}%
   {Dstar product of rcd linear map over scalar}%
\Index%73%S%RCstarS,RCstarT- линейное отображение векторных пространств
   {$(\RCstar S,\RCstar T)$\Hyph линейное отображение векторных пространств}%
   {rcs rct linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%586%S%star A- product of Astar linear map over scalar
   {$\star A$\Hyph произведением $A\star$\Hyph линейного отображения на скаляр}%
   {starA product of Astar linear map over scalar}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%683%S%star A- произведение Acr линейного отображения на скаляр
   {$\star A$\Hyph произведение \Acr линейного отображения на скаляр}%
   {starA product of Acr linear map over scalar}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%674%S%starA- произведение вектора на скаляр
   {$\star A$\Hyph произведение вектора на скаляр}%
   {starA product of vector over scalar, starA module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%192%S%starD- векторное пространство
   {$\star D$\Hyph векторное пространство}%
   {starD vector space}%
\Index%75%S%starD компонента координат вектора \Vector r
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%82%S%starT- представление Omega1 алгебры A в Omega2 алгебре M
   {\sT представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%90%T%Tstar- представление Omega1 алгебры A в Omega2 алгебре M
   {\Ts представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%689%Б%базис A- модуля
   {базис $A$\Hyph модуля}%
   {basis of A module}%
\Index%766%Б%базис ACRcirc модуля
   {базис $A\CRcirc$\Hyph модуля}%
   {basis of ACRcirc module}%
\Index%767%Б%базис CRcircA модуля
   {базис $\RCcirc A$\Hyph модуля}%
   {basis of CRcircA module}%
\Index%16%Б%базис drc векторного пространства r строк
   {базис \drc векторного пространства \subs строк}%
   {basis, r rows drc vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%197%Б%базис в D векторном пространстве
   {базис в $D$\Hyph векторном пространстве}%
   {basis, D vector space}%
\Index%24%Б%базис в rcd векторном пространстве
   {базис в \rcd векторном пространстве}%
   {basis, rcd vector space}%
\Index%25%Б%базис в rcd векторном пространстве c строк
   {базис в \rcd векторном пространстве \sups строк}%
   {basis, c rows rcd vector space}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%117%Б%базовый вектор представления группы Ли
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index%123%В%вектор Килинга второго рода
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index%782%В%вектор отображения
   {вектор отображения}%
   {vector of mapping}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%793%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%799%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%157%Д%дифференциал Гато отображения
   {дифференциал Гато отображения}%
   {Gateaux differential of map}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%662%З%закон ассоциативности для Astar- модуля
   {закон ассоциативности для $A\star$\Hyph модуля}%
   {associative law, Astar module over algebra}%
\Index%654%З%закон ассоциативности для D- модуля
   {закон ассоциативности для $D$\Hyph модуля}%
   {associative law, D module}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%161%З%закон ассоциативности для rcd линейных отображений векторных пространств
   {закон ассоциативности для \rcd линейных отображений векторных пространств}%
   {associative law for rcd linear maps of vector spaces}%
\Index%671%З%закон ассоциативности для starA- модуля
   {закон ассоциативности для $\star A$\Hyph модуля}%
   {associative law, starA module over algebra}%
\Index%501%З%закон ассоциативности для starD- векторного пространства
   {закон ассоциативности для $\star D$\Hyph векторного пространства}%
   {associative law, starD vector space}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%663%З%закон дистрибутивности для Astar- модуля
   {закон дистрибутивности для $A\star$\Hyph модуля}%
   {distributive law, Astar module over algebra}%
\Index%655%З%закон дистрибутивности для D- модуля
   {закон дистрибутивности для $D$\Hyph модуля}%
   {distributive law, D module}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%672%З%закон дистрибутивности для starA- модуля
   {закон дистрибутивности для $\star A$\Hyph модуля}%
   {distributive law, starA module over algebra}%
\Index%625%З%закон дистрибутивности для starD- векторного пространства
   {закон дистрибутивности для $\star D$\Hyph векторного пространства}%
   {distributive law, starD vector space}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%664%З%закон унитарности для Astar- модуля
   {закон унитарности для $A\star$\Hyph модуля}%
   {unitarity law, Astar module over algebra}%
\Index%656%З%закон унитарности для D- модуля
   {закон унитарности для $D$\Hyph модуля}%
   {unitarity law, D module}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\Index%673%З%закон унитарности для starA- модуля
   {закон унитарности для $\star A$\Hyph модуля}%
   {unitarity law, starA module over algebra}%
\Index%199%З%закон унитарности для starD- векторного пространства
   {закон унитарности для $\star D$\Hyph векторного пространства}%
   {unitarity law, starD vector space}%
\SetIndexSpace%
\Index%796%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений Omega1 алгебры A
   {категория \Ts представлений $\Omega$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%К%категория Tstar- представлений Omega1 алгебры из категории A
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%800%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%741%К%кватернионная алгебра
   {кватернионная алгебра}%
   {quaternion algebra}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный rcd изоморфизм
   {координатный \rcd изоморфизм}%
   {coordinate rcd isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%792%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%795%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль нaд кольцом
   {левый модуль нaд кольцом $D$}%
   {left module over ring}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг R- модуля
   {левый сдвиг $R$\Hyph модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%88%Л%линейная комбинация векторов
   {линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index%686%Л%линейная комбинация векторов A- модуля
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Index%98%Л%линейнное отображение тела, порождённое отображением G
   {линейное отображение тела, порождённое отображением $G$}%
   {linear map generated by map, division ring}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%21%Л%линейно зависимые векторы
   {линейно зависимые векторы}%
   {linearly dependent vectors}%
\Index%687%Л%линейно независимое множество A- модуля
   {линейно независимое множество $A$\Hyph модуля}%
   {linear independent vectors, module}%
\Index%34%Л%линейно независимые векторы
   {линейно независимые векторы}%
   {linearly independent vectors}%
\Index%613%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%398%Л%линейное отображение D векторных пространств
   {линейное отображение $D$\Hyph векторных пространств}%
   {linear map of D vector spaces}%
\Index%242%Л%линейное отображение D- векторных пространств над полем F
   {линейное отображение $D$\Hyph векторных пространств над полем $F$}%
   {linear map over field, vector space}%
\Index%35%Л%линейное отображение rcd векторных пространств
   {линейное отображение \rcd векторных пространств}%
   {linear map of rcd vector spaces}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear mapping of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%682%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {Linear Representation of Lie Group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%397%Л%линейный функционал на D модуле
   {линейный функционал на $D$\Hyph модуле}%
   {linear functional, D module}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor, algebra}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map, division ring}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%608%О%однородное линейное представление группы Ли
   {однородное линейное представление группы Ли}%
   {homogeneous Linear Representation of Lie Group}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%684%П%парные представления D- алгебры
   {парные представления $D$\Hyph алгебры}%
   {twin representations of D algebra}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное starT- представление
   {пассивное \sT представление}%
   {passive starT representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%794%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%797%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль нaд кольцом
   {правый модуль нaд кольцом $D$}%
   {right module over ring}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%271%П%произведение отображения на скаляр
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%781%С%скаляр отображения
   {скаляр отображения}%
   {scalar of mapping}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%459%С%стандартная компонента квадратичного отображения f над полем F
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты rcd базиса
   {стандартные координаты \rcd базиса}%
   {standard coordinates of rcd basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%475%С%сумма rcd линейных отображений
   {сумма \rcd линейных отображений}%
   {sum of rcd linear maps, rcd vector spaces}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%351%С%сумма линейных отображений
   {сумма линейных отображений}%
   {sum of linear maps}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%652%Т%тензорная степень алгебры
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Index%763%Т%тензорная степень представления
   {тензорная степень представления}%
   {tensor power of representation}%
\Index%195%Т%тензорная степень тела
   {тензорная степень тела $D$}%
   {tensor power of division ring}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%207%Т%тензорное произведение векторных пространств
   {тензорное произведение векторных пространств}%
   {tensor product of vector spaces}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%762%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Килинга
   {уравнение Килинга}%
   {Killing equation}%
\Index%494%У%уравнение Килинга второго рода
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%798%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%510%Ч%частная crd производная Гато отображения fb по переменной xa
   {частная \crd производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial crd derivative of map with respect to variable, D vector space}%
\Index%511%Ч%частная drc производная Гато отображения f^b по переменной x^a
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%513%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%500%Э%эффективное Tstar представление Omega- алгебры A
   {эффективное \Ts представление $\Omega$\Hyph алгебры $A$}%
   {effective Tstar representation of algebra}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление Omega- алгебры A
   {эффективное представление $\Omega$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%

\CloseIndex


==> Preface.BVector.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Preface}

\section{Preface}

Let $D$ be commutative ring of characteristic $0$.
In this book, I consider free $D$\Hyph module
which has countable basis.
The difference between a countable basis and a finite one is that
not any linear composition of vectors makes sense.

To explain this statement we assume that
$D$\Hyph module $A$ with countable basis $\Basis e$
is normed $D$\Hyph module.
If we drop requirement that expansion
\ShowEq{a=ai ei}
of vector $a$ relative to the basis $\Basis e$
is convergent series,
then we break out topology generated by the norm.
If a norm in $D$\Hyph module is not defined,
then we do not have a tool which allows us to identify
vector and its expansion relative to the basis
when all coefficients are different from $0$.

So, if $D$\Hyph module has countable basis,
then we consider two possibilities.
If we do not care for topology of $D$\Hyph module,
then we consider Hamel basis
(the definition
\ref{definition: module, Hamel basis}).
If norm is defined in $D$\Hyph module,
then we consider Schauder basis
(the definition
\ref{definition: Schauder basis}).

However in case of Schauder basis,
the request of convergence of the expansion of vector relative to basis
is not always sufficient. When we study a linear map,
we consider vectors
whose expansion in the basis
converges normally.



==> Preface.BVector.Eq.tex <==
%auto-ignore

\DefEq
{
\[a=a^{\gi i}e_{\gi i}\]
}
{a=ai ei}




==> Preface.BVector.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Предисловие}

\section{Предисловие}

Пусть $D$ - коммутативное кольцо характеристики $0$.
В этой книге я рассматриваю свободный $D$\Hyph модуль,
который имеет счётный базис.
Отличие счётного базиса от конечного состоит в том,
что не любая линейная композиция векторов имеет смысл.

Чтобы пояснить это утверждение, предположим, что
$D$\Hyph модуль $A$ со счётным базисом $\Basis e$
является нормированным $D$\Hyph модулем.
Если отказаться от требования, что разложение
\ShowEq{a=ai ei}
вектора $a$ относительно базиса $\Basis e$
является сходящимся рядом,
то мы разрушаем топологию, порождённую нормой.
Если норма в $D$\Hyph модуле не определена,
то у нас нет инструмента, позволяющего отождествить
вектор и его разложение относительно базиса,
если все коэффициенты отличны от $0$.

Поэтому, если $D$\Hyph модуль имеет счётный базис,
то мы рассматриваем две возможности.
Если нас не интересует топология $D$\Hyph модуля,
то мы рассматриваем базис Гамеля
(определение
\ref{definition: module, Hamel basis}).
Если норма определена в $D$\Hyph модуле,
то мы рассматриваем базис Шаудера
(определение
\ref{definition: Schauder basis}).

Однако в случае базиса Шаудера,
требование сходимости разложения вектора относительно базиса
не всегда достаточно. При изучении линейного отображения
мы рассматриваем векторы, разложение
которых относительно базиса
сходится нормально.


==> Schauder.Basis.Russian.tex <==
%auto-ignore
\input{Schauder.Basis.Eq}
\ifx\PrintBook\Defined
\chapter{Базис Шаудера}
\fi

\section{Топологическое кольцо}

\Input{Center.Ring}

\begin{definition}
Кольцо $D$ называется 
\AddIndex{топологическим кольцом}{topological ring}\footnote{Определение
дано согласно
определению из \citeBib{Pontryagin: Topological Group},
глава 4},
если $D$ является топологическим пространством, и алгебраические операции,
определённые в $D$, непрерывны в топологическом пространстве $D$.
\qed
\end{definition}

Согласно определению, для произвольных элементов $a, b\in D$
и для произвольных окрестностей $W_{a-b}$ элемента $a-b$,
$W_{ab}$ элемента $ab$ существуют такие окрестности $W_a$
элемента $a$ и $W_b$ элемента $b$, что $W_a-W_b\subset W_{a-b}$,
$W_aW_b\subset W_{ab}$.

\begin{definition}
\label{definition: norm on ring}
\AddIndex{Норма на кольце}
{norm on ring} $D$\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2, а также согласно
определению \citeBib{Arnautov Glavatsky Mikhalev}-1.1.12,
с. 23.} - это отображение
\[d\in D\rightarrow |d|\in R\]
такое, что
\begin{itemize}
\item $|a|\ge 0$
\item $|a|=0$ равносильно $a=0$
\item $|ab|=|a|\ |b|$
\item $|a+b|\le|a|+|b|$
\end{itemize}

Кольцо $D$, наделённое структурой, определяемой заданием на
$D$ нормы, называется \AddIndex{нормированным кольцом}{normed ring}.
\qed
\end{definition}

Инвариантное расстояние на аддитивной группе кольца $D$
\[d(a,b)=|a-b|\]
определяет топологию метрического пространства,
согласующуюся со структурой кольца в $D$.

\begin{definition}
\label{definition: limit of sequence, normed ring}
Пусть $D$ - нормированное кольцо.
Элемент $a\in D$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
$\{a_n\}$
\ShowEq{limit of sequence, normed ring}
если для любого $\epsilon\in R$, $\epsilon>0$
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что $|a_n-a|<\epsilon$ для любого $n>n_0$.
\qed
\end{definition}

\begin{definition}
Пусть $D$ - нормированное кольцо.
Последовательность $\{a_n\}$, $a_n\in D$ называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого $\epsilon\in R$, $\epsilon>0$,
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что $|a_p-a_q|<\epsilon$ для любых $p$, $q>n_0$.
\qed
\end{definition}

\begin{definition}
Нормированное кольцо $D$ называется 
\AddIndex{полным}{complete ring}
если любая фундаментальная последовательность элементов
данного кольца сходится, т. е.
имеет предел в этом кольце.
\qed
\end{definition}

Пусть $D$ - полное кольцо характеристики $0$.
Так как операция деления в кольце, вообще говоря, не определена,
мы не можем утверждать, что кольцо $D$ содержит подполе
рациональных чисел.
Мы будем полагать, что рассматриваемое кольцо $D$ содержит
поле рациональных чисел.
При этом очевидно, что кольцо имеет характеристику $0$.

\begin{theorem}
Пусть $D$ - кольцо, содержащее
поле рациональных чисел, и пусть $d\in D$.
Тогда для любого целого числа $n\in Z$
\ShowEq{inverse integer in ring}
\end{theorem}
\begin{proof}
Согласно теореме \ref{theorem: integer subring of ring}
справедлива цепочка равенств
\ShowEq{inverse integer in ring, 1}
Умножив правую и левую части равенства
\EqRef{inverse integer in ring, 1} на $n^{-1}$,
получим
\ShowEq{inverse integer in ring, 2}
Из \EqRef{inverse integer in ring, 2} следует
\EqRef{inverse integer in ring}.
\end{proof}

\begin{theorem}
\label{theorem: ring, rational number}
Пусть $D$ - кольцо, содержащее
поле рациональных чисел, и пусть $d\in D$.
Тогда любое рациональное число $p\in Q$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Мы можем представить рациональное число $p\in Q$ в
виде $p=mn^{-1}$, $m$, $n\in Z$.
Утверждение теоремы следует из цепочки равенств
\[
pd=mn^{-1}d=n^{-1}dm=dmn^{-1}=dp
\]
основанной на утверждении теоремы \ref{theorem: integer subring of ring}
и равенстве \EqRef{inverse integer in ring}.
\end{proof}

\begin{theorem}
\label{theorem: rational subring of center}
Пусть $D$ - кольцо, содержащее
поле рациональных чисел.
Тогда поле рациональных чисел $Q$ является подполем центра $Z(D)$ кольца $D$.
\end{theorem}
\begin{proof}
Следствие теоремы \ref{theorem: ring, rational number}.
\end{proof}

В дальнейшем, говоря о нормированном кольце характеристики $0$,
мы будем предполагать, что определён гомеоморфизм поля рациональных
чисел $Q$ в кольцо $D$.

\begin{theorem}
\label{theorem: limit of sequence, normed ring, product on scalar}
Пусть $D$ - нормированное кольцо характеристики $0$ и пусть $d\in D$.
Пусть $a\in D$ - предел последовательности $\{a_n\}$.
Тогда
\[
\lim_{n\rightarrow\infty}(a_nd)=ad
\]
\[
\lim_{n\rightarrow\infty}(da_n)=da
\]
\end{theorem}
\begin{proof}
Утверждение теоремы тривиально, однако я привожу доказательство
для полноты текста. 
Поскольку $a\in D$ - предел последовательности $\{a_n\}$,
то согласно определению
\ref{definition: limit of sequence, normed ring}
для заданного $\epsilon\in R$, $\epsilon>0$,
существует натуральное число $n_0$ такое, что
\ShowEq{an-a d}
для любого $n>n_0$.
Согласно определению \ref{definition: norm on ring}
утверждение теоремы следует из неравенств
\ShowEq{an-a d1}
для любого $n>n_0$.
\end{proof}

\begin{theorem}
\label{theorem: complete ring contains real number}
Полное кольцо $D$ характеристики $0$
содержит в качестве подполя изоморфный образ поля $R$
действительных чисел.
Это поле обычно отождествляют с $R$.
\end{theorem}
\begin{proof}
Рассмотрим фундаментальную последовательность рациональных чисел $\{p_n\}$.
Пусть $p'$ - предел этой последовательности в кольце $D$.
Пусть $p$ - предел этой последовательности в поле $R$.
Так как вложение поля $Q$ в тело $D$ гомеоморфно,
то мы можем отождествить $p'\in D$ и $p\in R$.
\end{proof}

\begin{theorem}
\label{theorem: complete ring and real number}
Пусть $D$ - полное кольцо характеристики $0$ и пусть $d\in D$.
Тогда любое действительное число $p\in R$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Мы можем представить действительное число $p\in R$ в
виде фундаментальной последовательности рациональных чисел $\{p_n\}$.
Утверждение теоремы следует из цепочки равенств
\ShowEq{complete ring and real number}
основанной на утверждении теоремы
\ref{theorem: limit of sequence, normed ring, product on scalar}.
\end{proof}

\section{Нормированная \texorpdfstring{$D$}{D}-алгебра}

\ifx\texFuture\Defined
\begin{definition}
Пусть $D$ - топологическое коммутативное кольцо.
$D$\Hyph алгебра $A$ называется 
\AddIndex{топологической $D$\Hyph алгеброй}
{topological D algebra}\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: Topological Vector Space},
с. 21},
если $A$ наделено топологией, согласующейся со
структурой аддитивной группы в $A$,
и отображения
\ShowEq{topological D algebra}
непрерывны.
\qed
\end{definition}
\fi

\begin{definition}
\label{definition: norm on D module}
Пусть $D$ - нормированое коммутативное кольцо.\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$3.
Для нормы мы пользуемся обозначением $|a|$ или $\|a\|$.
}
\AddIndex{Норма в $D$\Hyph модуле}
{norm on D module} $A$
 - это отображение
\ShowEq{norm on D module}
такое, что
\StartLabelItem{definition: norm on D module}
\begin{enumerate}
\ShowEq{norm on D module 1}
\ShowEq{norm on D module 2, 1}
равносильно
\ShowEq{norm on D module 2, 2}
\ShowEq{norm on D module 3}
\end{enumerate}
$D$\Hyph модуль $A$,
наделённый структурой, определяемой заданием на
$A$ нормы, называется
\AddIndex{нормированным $D$\Hyph модулем}{normed D module}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: normed module, norm of difference}
Норма в $D$\Hyph модуле $A$ удовлетворяет равенству
\ShowEq{normed module, norm of difference}
\end{theorem}
\begin{proof}
Из равенства
\ShowEq{normed module, norm of difference, 1}
и утверждения
\ref{item: norm on D module 3, 1}
следует
\ShowEq{normed module, norm of difference, 2}
Равенство
\EqRef{normed module, norm of difference}
следует из равенства
\EqRef{normed module, norm of difference, 2}.
\end{proof}

\begin{definition}
\label{definition: normal basis}
Базис $\Basis e$ называется
\AddIndex{нормированным базисом}{normal basis},
если
\ShowEq{Banach algebra, normal basis}
для любого вектора $e_{\gi i}$ базиса $\Basis e$.
\qed
\end{definition}

\begin{definition}
\label{definition: limit of sequence, normed module}
Пусть $A$ - нормированный $D$\Hyph модуль.
Элемент $a\in A$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
\ShowEq{limit of sequence, normed module}
если для любого $\epsilon\in R$, $\epsilon>0$
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\ShowEq{an-a}
для любого $n>n_0$.
\qed
\end{definition}

\begin{definition}
\label{definition: fundamental sequence, normed module}
Пусть $A$ - нормированный $D$\Hyph модуль.
Последовательность $\{a_n\}$, $a_n\in A$, называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого $\epsilon\in R$, $\epsilon>0$,
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что 
\ShowEq{ap-aq}
для любых $p$, $q>n_0$.
\qed
\end{definition}

\begin{definition}
Нормированный $D$\Hyph модуль $A$ называется 
\AddIndex{банаховым $D$\Hyph модулем}{Banach module}
если любая фундаментальная последовательность элементов
модуля $A$ сходится, т. е.
имеет предел в модуле $A$.
\qed
\end{definition}

\begin{definition}
\label{definition: norm on d algebra}
Пусть $D$ - нормированое коммутативное кольцо.
Пусть $A$ - $D$\Hyph алгебра.
Норма
\ShowEq{norm on d algebra}
в $D$\Hyph модуле $A$ такая, что
\ShowEq{norm on d algebra 3}
называется
\AddIndex{нормой в $D$\Hyph алгебре}
{norm on D algebra} $A$.
$D$\Hyph алгебра $A$,
наделённая структурой, определяемой заданием на
$A$ нормы, называется
\AddIndex{нормированной $D$\Hyph алгеброй}
{normed D algebra}.
\qed
\end{definition}

\begin{definition}
Нормированная $D$\Hyph алгебра $A$ называется 
\AddIndex{банаховой $D$\Hyph алгеброй}{Banach algebra}
если любая фундаментальная последовательность элементов
алгебры $A$ сходится, т. е.
имеет предел в алгебре $A$.
\qed
\end{definition}

\begin{definition}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Множество элементов
\ShowEq{unit sphere in algebra}
называется
\AddIndex{единичной сферой в алгебре}{unit sphere in algebra} $A$.
\qed
\end{definition}

\section{Нормированный \texorpdfstring{$D$\Hyph}{D-}модуль
\texorpdfstring{$\mathcal L(D;A_1;A_2)$}{Lc(D;A1;A2)}}
\label{section: Module L(D;A1;A2)}

\begin{definition}
\label{definition: continuous map, module}
Отображение
\ShowEq{f A1 A2}
$D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\DrawEq{continuous map, x}{}
влечёт
\DrawEq{continuous map, y}{}
\qed
\end{definition}

\begin{theorem}
Пусть\footnote{Эта теорема написана
на основе похожей теоремы,
\citeBib{Kolmogorov Fomin}, страница 174.}
\ShowEq{f A1 A2}
линейное отображение
$D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$.
Если линейное отображение $f$ непрерывно в $x\in A_1$,
то линейное отображение $f$ непрерывно всюду на $D$\Hyph модуле $A_1$.
\end{theorem}
\begin{proof}
Пусть $\epsilon>0$.
Согласно определению
\ref{definition: continuous map, module},
существует такое $\delta>0$, что
\DrawEq{continuous map, x}{at x}
влечёт
\ShowEq{continuous map, y at x}
Пусть $b\in A_1$.
Из равенства
\eqRef{continuous map, x}{at x}
следует
\ShowEq{continuous map, x 1}
Из равенства
\EqRef{continuous map, y at x}
следует
\ShowEq{continuous map, y 1}
Следовательно, линейное отображение $f$ непрерывно
в точке $x+b$.
\end{proof}

\begin{corollary}
\label{corollary: linear map is continuous at 0}
Линейное отображение
\ShowEq{f A1 A2}
нормированного $D$\Hyph модуля $A_1$
в нормированный $D$\Hyph модуль $A_2$
непрерывно тогда и только тогда, если оно непрерывно в точке $0\in A_1$.
\qed
\end{corollary}

\begin{theorem}
\label{theorem: sum of continuous linear maps}
Сумма непрерывных линейных отображений
$D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$
является непрерывным линейным отображением.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{f A1 A2}
непрерывное линейное отображение.
Согласно следствию
\ref{corollary: linear map is continuous at 0}
и определению
\ref{definition: continuous map, module},
для заданного $\epsilon>0$
существует такое $\delta_1>0$, что
\ShowEq{continuous map, x, 1}
влечёт
\ShowEq{continuous map, y, 1}
Пусть
\ShowEq{g A1 A2}
непрерывное линейное отображение.
Согласно следствию
\ref{corollary: linear map is continuous at 0}
и определению
\ref{definition: continuous map, module},
для заданного $\epsilon>0$
существует такое $\delta_2>0$, что
\ShowEq{continuous map, x, 2}
влечёт
\ShowEq{continuous map, y, 2}
Пусть
\ShowEq{delta 1 2}
Из неравенств
\EqRef{continuous map, y, 1},
\EqRef{continuous map, y, 2}
и утверждения
\ref{item: norm on D module 3, 1}
следует, что
\ShowEq{continuous map, x, 3}
влечёт
\ShowEq{continuous map, y, 3}
Следовательно,
согласно следствию
\ref{corollary: linear map is continuous at 0}
и определению
\ref{definition: continuous map, module},
линейное отображение $f+g$ непрерывно.
\end{proof}

\begin{theorem}
\label{theorem: Product of continuous map over scalar}
Пусть
\ShowEq{f A1 A2}
непрерывное линейное отображение
$D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$.
Произведение отображения $f$
на скаляр $d\in D$
является непрерывным линейным отображением.
\end{theorem}
\begin{proof}
Согласно следствию
\ref{corollary: linear map is continuous at 0}
и определению
\ref{definition: continuous map, module},
для заданного $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{continuous map, x, 3}
влечёт
\ShowEq{continuous map, y, d}
Из неравенства
\EqRef{continuous map, y, d}
и утверждения
\ref{item: norm on D module 3, 2},
следует, что
\ShowEq{continuous map, x, 3}
влечёт
\ShowEq{continuous map, y, 4}
Следовательно,
согласно следствию
\ref{corollary: linear map is continuous at 0}
и определению
\ref{definition: continuous map, module},
линейное отображение $d\,f$ непрерывно.
\end{proof}

\begin{theorem}
Множество
\ShowEq{set continuous linear maps, module}
непрерывных линейных отображений
нормированного $D$\Hyph модуля $A_1$
в нормированный $D$\Hyph модуль $A_2$
является $D$\Hyph модулем.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\ref{theorem: sum of continuous linear maps},
\ref{theorem: Product of continuous map over scalar}.
\end{proof}

\begin{theorem}
\label{theorem: norm of map, module}
Пусть $A_1$ - $D$\Hyph модуль с нормой $\|x\|_1$.
Пусть $A_2$ - $D$\Hyph модуль с нормой $\|y\|_2$.
Отображение
\ShowEq{LDA->R}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, module}
является нормой $D$\Hyph модуля $\LDA$
и называется
\AddIndex{нормой отображения $f$}{norm of map}.
\end{theorem}
\begin{proof}
Утверждение
\ref{item: norm on D module 1}
очевидно.

Пусть $\|f\|=0$.
Согласно определению
\EqRef{norm of map, module}
\ShowEq{|f|=0 1}
для любого $x\in A_1$.
Согласно утверждению
\ref{item: norm on D module 2},
\ShowEq{|f|=0 2}
для любого $x\in A_1$.
Следовательно, утверждение
\ref{item: norm on D module 2}
верно для $\|f\|$.

Согласно определению
\EqRef{sum of linear maps, definition}
и утверждению
\ref{item: norm on D module 3, 1},
\ShowEq{|f1+f2| 1}
Из неравенства
\EqRef{|f1+f2| 1}
и определения
\EqRef{norm of map, module}
следует
\ShowEq{|f1+f2| 2}
Следовательно, утверждение
\ref{item: norm on D module 3, 1}
верно для $\|f\|$.

Согласно определению
\EqRef{product of map over scalar, definition}
и утверждению
\ref{item: norm on D module 3, 2},
\ShowEq{|df| 1}
Из неравенства
\EqRef{|df| 1}
и определения
\EqRef{norm of map, module}
следует
\ShowEq{|df| 2}
Следовательно, утверждение
\ref{item: norm on D module 3, 2}
верно для $\|f\|$.
\end{proof}

\begin{theorem}
Пусть $D$ - кольцо с нормой $|d|$.
Пусть $A$ - $D$\Hyph модуль с нормой $\|x\|_0$.
Отображение
\ShowEq{A'->R}
определённое равенством
\ShowEq{norm of functional}
является нормой $D$\Hyph модуля $A'$
и называется
\AddIndex{нормой функционала}{norm of functional} $f$.
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: norm of map, module}.
\end{proof}

\begin{theorem}
Пусть $D$ - кольцо с нормой $|d|$.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$ с нормой $\|x\|_1$.
Пусть $A'$ - сопряжённый $D$\Hyph модуль с нормой $\|x\|_2$.
Тогда
\ShowEq{norm of conjugate basis}
\end{theorem}
\begin{proof}
Пусть индекс $\gi i$ имеет заданное значение.
Пусть $a\in A$.
Так как
\ShowEq{a=a-+ai}
то согласно утверждению
\ref{item: norm on D module 3, 1}
\ShowEq{a=a-+ai 1}
Если
\ShowEq{a=a-+ai 2}
то согласно утверждениям
\ref{item: norm on D module 2},
\ref{item: norm on D module 3, 2}
\ShowEq{a=a-+ai 3}
Следовательно,
\ShowEq{a=a-+ai 4}
Равенство
\EqRef{norm of conjugate basis}
следует из равенства
\EqRef{a=a-+ai 4}.
\end{proof}

\begin{corollary}
\label{corollary: basis dual to normal basis is normal}
Пусть $\Basis e$ - нормированный базис нормированного $D$\Hyph модуля $A$.
Базис, двойственный базису $\Basis e$,
также является нормированным базисом нормированного $D$\Hyph модуля $A'$.
\qed
\end{corollary}

\begin{theorem}
Пусть $\Basis e_1$ - базис $D$\Hyph модуля $A_1$ с нормой $\|x\|_1$.
Пусть $\Basis e_2$ - базис $D$\Hyph модуля $A_2$ с нормой $\|x\|_2$.
Тогда
\ShowEq{norm of basis L(A1,A2)}
\end{theorem}
\begin{proof}
Пусть индексы $\gi i$, $\gi j$ имеют заданные значения.
Пусть $a\in A_1$.
Так как
\ShowEq{a=a-+ai L(A1,A2)}
то согласно утверждению
\ref{item: norm on D module 3, 1}
\ShowEq{a=a-+ai 1 L(A1,A2)}
Если
\ShowEq{a=a-+ai 2 L(A1,A2)}
то согласно утверждениям
\ref{item: norm on D module 2},
\ref{item: norm on D module 3, 2}
\ShowEq{a=a-+ai 3 L(A1,A2)}
Так как
\ShowEq{a=a-+ai 5}
то согласно утверждению
\ref{item: norm on D module 3, 2}
\ShowEq{a=a-+ai 6}
Из равенств
\EqRef{a=a-+ai 3 L(A1,A2)},
\EqRef{a=a-+ai 6}
следует
\ShowEq{a=a-+ai 7}
Равенство
\EqRef{norm of basis L(A1,A2)}
следует из равенства
\EqRef{a=a-+ai 7}.
\end{proof}

\begin{corollary}
\label{corollary: norm of basis L(A1,A2)}
Пусть $\Basis e_1$
- нормированный базис $D$\Hyph модуля $A_1$ с нормой $\|x\|_1$.
Пусть $\Basis e_2$
- нормированный базис $D$\Hyph модуля $A_2$ с нормой $\|x\|_2$.
Тогда
\ShowEq{normal basis L(A1,A2)}
\qed
\end{corollary}

\begin{theorem}
\label{theorem: norm of linear map, module}
Пусть
\ShowEq{f A1 A2}
линейное отображение $D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$.
Тогда
\ShowEq{norm of linear map, module}
\end{theorem}
\begin{proof}
Из определения
\ref{definition: linear map from A1 to A2, module}
и теорем
\ref{theorem: complete ring contains real number},
\ref{theorem: complete ring and real number}
следует
\ShowEq{linear map and real number}
Из равенства \EqRef{linear map and real number}
и утверждения \ref{item: norm on D module 3, 2}
следует
\ShowEq{linear map and real number, 1}
Полагая $\displaystyle r=\frac 1{\|x\|_1}$, мы получим
\ShowEq{norm of linear map, module, 1}
Равенство \EqRef{norm of linear map, module}
следует из равенств \EqRef{norm of linear map, module, 1}
и \EqRef{norm of map, module}.
\end{proof}

\begin{theorem}
\label{theorem: |fx|<|f||x|}
Пусть
\ShowEq{f A1 A2}
линейное отображение $D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$.
Тогда
\ShowEq{|fx|<|f||x|}
\end{theorem}
\begin{proof}
Согласно утверждению
\ref{item: norm on D module 3, 2}
\ShowEq{x/|x|}
Из теоремы
\ref{theorem: norm of linear map, module}
и равенства
\EqRef{x/|x|}
следует
\ShowEq{f x/|x|}
Из утверждения
\ref{item: norm on D module 3, 2}
и равенства
\EqRef{f x/|x|}
следует
\ShowEq{f x/|x| 1}
Неравенство
\EqRef{|fx|<|f||x|}
следует из неравенства
\EqRef{f x/|x| 1}.
\end{proof}

\begin{theorem}
\label{theorem: map is continuous iff}
Пусть\footnote{Эта теорема написана
на основе теорем, рассмотренных в
\citeBib{Kolmogorov Fomin}, страницы 174 - 176.}
\ShowEq{f A1 A2}
линейное отображение $D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$.
Отображение $f$ непрерывно тогда и только тогда, когда
\ShowEq{|f|<infty}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{|f|<infty}
Поскольку отображение $f$ линейно, то
согласно теореме \ref{theorem: norm of map, module}
\ShowEq{|f|<infty 1}
Возьмём произвольное $\epsilon>0$. Положим $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Тогда из неравенства
\ShowEq{|f|<infty 2}
следует
\ShowEq{|f|<infty 3}
Согласно определению \ref{definition: continuous map, module}
отображение $f$ непрерывно.

Пусть
\ShowEq{|f|=infty}
Согласно теореме
\ref{theorem: norm of map, module},
для любого $n$ существует $x_n$ такое, что
\ShowEq{|f(x)|>n}
Положим
\ShowEq{xn=}
Согласно определению
\ref{definition: linear map from A1 to A2, algebra},
утверждению \ref{item: norm on D module 3, 2},
равенству
\EqRef{xn=},
неравенству
\EqRef{|f(x)|>n}
\ShowEq{|f(y)|=1}
Следовательно, отображение $f$ не является непрерывным в точке $0\in A_1$.
\end{proof}

$D$\Hyph модуль $\LcDA$ является подмодулем
$D$\Hyph модуля $\LDA$.
Согласно теореме
\ref{theorem: map is continuous iff},
если
\ShowEq{LcDA-LDA}
то
\ShowEq{|f|=infty}

\ifx\texFuture\Defined
\begin{theorem}
Пусть $A_1$ - $D$\Hyph модуль с нормой $\|x\|_1$.
Пусть $A_2$ - банахов $D$\Hyph модуль с нормой $\|y\|_2$.
$D$\Hyph модуль $\LcDA$ является банаховым $D$\Hyph модулем.
\end{theorem}
\begin{proof}
\end{proof}
\fi

\begin{theorem}
\label{theorem: norm of product of maps}
Пусть $A_1$ - $D$\Hyph модуль с нормой $\|x\|_1$.
Пусть $A_2$ - $D$\Hyph модуль с нормой $\|x\|_2$.
Пусть $A_3$ - $D$\Hyph модуль с нормой $\|x\|_3$.
Пусть
\ShowEq{g A1 A2}
\ShowEq{f A2 A3}
непрерывные линейные отображения.
Отображение
\ShowEq{fg}
является непрерывным линейным отображением
\ShowEq{|fg|}
\end{theorem}
\begin{proof}
Согласно определениям
\EqRef{(fg)a=f(ga)},
\EqRef{norm of map, module}\footnote{Пусть
\ShowEq{fi A1 R}
Вообще говоря, отображения $f_1$, $f_2$ имеют максимум
в различных точках множества $A_1$.
Следовательно,
\ShowEq{fi A1 R 1}
}
\ShowEq{|fg| 1}
Так как, вообще говоря,
\ShowEq{g A1}
то
\ShowEq{|fg| 0}
Из неравенств
\EqRef{|fg| 1},
\EqRef{|fg| 0}
следует
\ShowEq{|fg| 2}
Неравенство
\EqRef{|fg|}
следует из неравенства
\EqRef{|fg| 2}
и определения
\EqRef{norm of map, module}.
%и утверждению
%\ref{item: norm on d algebra 3, 2},
\end{proof}

\begin{theorem}
Нормированный $D$\Hyph модуль $\mathcal{LC}(D;A;A)$
является нормированной $D$\Hyph алгеброй,
в которой произведение определено согласно правилу
\ShowEq{f g ->}
\end{theorem}
\begin{proof}
Доказательство утверждения, что $D$\Hyph модуль $\mathcal{LC}(D;A;A)$
является $D$\Hyph алгеброй, аналогично доказательству теоремы
\xRef{8433-5163}{theorem: module L(A;A) is algebra}.
Согласно определению
\ref{definition: norm on d algebra}
и теореме
\ref{theorem: norm of product of maps},
норма
\EqRef{norm of map, module}
является нормой на $D$\Hyph алгебре $\mathcal{LC}(D;A;A)$.
\end{proof}

\section{Нормированный \texorpdfstring{$D$\Hyph}{D-}модуль
\texorpdfstring{$\mathcal L(D;A_1,...,A_n;A)$}{L(D;A1,...,An;A)}}
\label{section: Module L(D;A1,...,An;A)}

\begin{definition}
\label{definition: continuous multivariable map, module}
Пусть
\ShowEq{Ai 1n}
- банахова $D$\Hyph алгебра с нормой $\|x\|_i$.
Пусть $A$
- банахова $D$\Hyph алгебра с нормой $\|x\|$.
Отображение нескольких переменных
\ShowEq{A1...An->A}
называется \AddIndex{непрерывным}{continuous multivariable map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\DrawEq{|xi|<e, 1-n}{}
влечёт
\DrawEq{continuous multivariable map, y}{}
\qed
\end{definition}

\begin{theorem}
\label{theorem: sum of continuous multivariable maps}
Сумма непрерывных отображений нескольких переменных
является непрерывным отображением нескольких переменных.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{A1...An->A}
непрерывное отображение нескольких переменных.
Согласно определению
\ref{definition: continuous multivariable map, module},
для заданного $\epsilon>0$
существует такое $\delta_1>0$, что
\ShowEq{continuous multivariable map, x, 1}
влечёт
\ShowEq{continuous multivariable map, y, 1}
Пусть
\ShowEq{g A1...An->A}
непрерывное отображение нескольких переменных.
Согласно определению
\ref{definition: continuous multivariable map, module},
для заданного $\epsilon>0$
существует такое $\delta_2>0$, что
\ShowEq{continuous multivariable map, x, 2}
влечёт
\ShowEq{continuous multivariable map, y, 2}
Пусть
\ShowEq{delta 1 2}
Из неравенств
\EqRef{continuous multivariable map, y, 1},
\EqRef{continuous multivariable map, y, 2}
и утверждения
\ref{item: norm on D module 3, 1},
следует, что
\ShowEq{continuous multivariable map, x, 3}
влечёт
\ShowEq{continuous multivariable map, y, 3}
Следовательно,
согласно определению
\ref{definition: continuous multivariable map, module},
отображение нескольких переменных $f+g$ непрерывно.
\end{proof}

\begin{theorem}
\label{theorem: sum of continuous polylinear maps}
Сумма непрерывных полилинейных отображений
является непрерывным полилинейным отображением.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из теорем
\xRef{1011.3102}{theorem: sum of polylinear maps, algebra},
\ref{theorem: sum of continuous multivariable maps}.
\end{proof}

\begin{theorem}
\label{theorem: Product of continuous multivariable map over scalar}
Произведение непрерывного отображения $f$ нескольких переменных
на скаляр $d\in D$
является непрерывным отображением нескольких переменных.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{A1...An->A}
непрерывное отображение нескольких переменных.
Согласно определению
\ref{definition: continuous multivariable map, module},
для заданного $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{continuous multivariable map, x, 3}
влечёт
\ShowEq{continuous multivariable map, y, d}
Из неравенства
\EqRef{continuous multivariable map, y, d}
и утверждения
\ref{item: norm on D module 3, 2},
следует, что
\ShowEq{continuous multivariable map, x, 3}
влечёт
\ShowEq{continuous multivariable map, y, 4}
Следовательно,
согласно определению
\ref{definition: continuous multivariable map, module},
отображение $d\,f$ непрерывно.
\end{proof}

\begin{theorem}
\label{theorem: Product of continuous polylinear map over scalar}
Произведение непрерывного полилинейного отображения $f$
на скаляр $d\in D$
является непрерывным полилинейным отображением.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из теорем
\xRef{1011.3102}{theorem: polylinear map times scalar, algebra},
\ref{theorem: Product of continuous multivariable map over scalar}.
\end{proof}

\begin{theorem}
Множество
\ShowEq{set continuous multivariable maps, module}
непрерывных отображений нескольких переменных
является $D$\Hyph модулем.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\ref{theorem: sum of continuous multivariable maps},
\ref{theorem: Product of continuous multivariable map over scalar}.
\end{proof}

\begin{theorem}
Множество
\ShowEq{set continuous polylinear maps, module}
непрерывных полилинейных отображений
является $D$\Hyph модулем.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\ref{theorem: sum of continuous polylinear maps},
\ref{theorem: Product of continuous polylinear map over scalar}.
\end{proof}

Пусть $A_1$ - $D$\Hyph модуль с нормой $\|x\|_1$.
Пусть $A_2$ - $D$\Hyph модуль с нормой $\|x\|_2$.
Пусть $A_3$ - $D$\Hyph модуль с нормой $\|x\|_3$.
Так как $\mathcal L(D;A_2;A_3)$ - $D$\Hyph модуль с нормой
\ShowEq{|f|23}
то мы можем рассмотреть непрерывное отображение
\ShowEq{h A1 A2->A3}
Если $a_1\in A_1$, то
\ShowEq{h a_1}
непрерывное отображение.
Согласно теореме
\ref{theorem: |fx|<|f||x|}
\ShowEq{|a3|=|ha1||a2|}
Так как
\ShowEq{L(A1,L(A2,A3))}
нормированный $D$\Hyph модуль,
то согласно теореме
\ref{theorem: |fx|<|f||x|}
\ShowEq{|ha1|}
Из неравенств
\EqRef{|a3|=|ha1||a2|},
\EqRef{|ha1|}
следует
\ShowEq{a3 h a1 a2}
Мы можем рассматривать отображение
\EqRef{h A1 A2->A3}
как билинейное отображение
\ShowEq{f A1,A2->A3}
определённое согласно правилу
\ShowEq{f a1,a2}
Опираясь на теоремы
\ref{theorem: norm of map, module},
\ref{theorem: |fx|<|f||x|}
и неравенство
\EqRef{a3 h a1 a2},
мы определим норму билинейного отображения $f$ равенством
\ShowEq{|f| a1a2}

Применяя индукцию по числу переменных,
мы можем обобщить определение
нормы билинейного отображения.

\begin{definition}
\label{definition: norm of polylinear map}
Пусть
\ShowEq{Ai 1n}
- банахова $D$\Hyph алгебра с нормой $\|x\|_i$.
Пусть $A$
- банахова $D$\Hyph алгебра с нормой $\|x\|$.
Пусть
\ShowEq{f A1...An->A}
- полилинейное отображение.
Величина
\ShowEq{norm of polymap, module}
называется
\AddIndex{нормой полилинейного отображения $f$}
{norm of polymap}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: norm of polylinear map, module}
Пусть
\ShowEq{Ai 1n}
- банахов $D$\Hyph модуль с нормой $\|x\|_i$.
Пусть $A$
- банахов $D$\Hyph модуль с нормой $\|x\|$.
Пусть
\ShowEq{f A1...An->A}
полилинейное отображение.
Тогда
\ShowEq{norm of polylinear map, module}
\end{theorem}
\begin{proof}
Из определения
\ref{definition: polylinear map of modules}
и теорем
\ref{theorem: complete ring contains real number},
\ref{theorem: complete ring and real number}
следует
\ShowEq{polylinear map and real number}
Из равенства \EqRef{polylinear map and real number}
и утверждения \ref{item: norm on D module 3, 2}
следует
\ShowEq{polylinear map and real number, 1}
Полагая $\displaystyle r=\frac 1{\|x\|_1}$, мы получим
\ShowEq{norm of polylinear map, module, 1}
Равенство \EqRef{norm of polylinear map, module}
следует из равенств \EqRef{norm of polylinear map, module, 1}
и \EqRef{norm of polymap, module}.
\end{proof}

\begin{theorem}
\label{theorem: |fx|<|f||x|1n}
Пусть
\ShowEq{Ai 1n}
- банахов $D$\Hyph модуль с нормой $\|x\|_i$.
Пусть $A$
- банахов $D$\Hyph модуль с нормой $\|x\|$.
Пусть
\ShowEq{f A1...An->A}
полилинейное отображение.
Тогда
\DrawEq{|fx|<|f||x|1n}{theorem}
\end{theorem}
\begin{proof}
Согласно утверждению
\ref{item: norm on D module 3, 2}
\ShowEq{x/|x|1n}
Из теоремы
\ref{theorem: norm of polylinear map, module}
и равенства
\EqRef{x/|x|1n}
следует
\ShowEq{f x/|x|1n}
Из утверждения
\ref{item: norm on D module 3, 2}
и равенства
\EqRef{f x/|x|1n}
следует
\ShowEq{f x/|x|1n 1}
Неравенство
\eqRef{|fx|<|f||x|1n}{theorem}
следует из неравенства
\EqRef{f x/|x|1n 1}.
\end{proof}

Пусть
\ShowEq{Ai 1n}
- банахов $D$\Hyph модуль с нормой $\|x\|_i$.
Пусть $A$
- банахов $D$\Hyph модуль с нормой $\|x\|$.
Мы можем представить полилинейное отображение
\ShowEq{f A1...An->A}
в следующем виде
\DrawEq{f1n=hx}{convention}
где
\ShowEq{h 1n-1->A}
полилинейное отображение.

\begin{theorem}
\label{theorem: polylinear map f h()}
Если отображение $f$ непрерывно, то отображение
\ShowEq{polymap 3, algebra}
также непрерывно.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: continuous multivariable map, module},
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\DrawEq{|xi|<e, 1-n}{}
влечёт
\ShowEq{polymap 30, y}
Следовательно,
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{polymap 3, x}
влечёт
\ShowEq{polymap 3, y}
Из равенства
\eqRef{f1n=hx}{convention}
и неравенства
\EqRef{polymap 3, y}
следует, что
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{polymap 3, x}
влечёт
\ShowEq{polymap 31, y}
Согласно определению
\ref{definition: continuous map, module},
отображение
\ShowEq{polymap 32, y}
непрерывно.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map f h}
Если отображение $f$ непрерывно, то отображение
$h$ также непрерывно.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: continuous multivariable map, module},
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\DrawEq{|xi|<e, 1-n}{}
влечёт
\ShowEq{polymap 30, y}
Следовательно,
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{polymap 4, x}
влечёт
\ShowEq{polymap 4, y}
Из равенства
\eqRef{f1n=hx}{convention}
и неравенства
\EqRef{polymap 4, y}
следует, что
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{polymap 4, x}
влечёт
\ShowEq{polymap 41, y}
Из неравенства
\EqRef{polymap 41, y}
следует, что
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{polymap 4, x}
влечёт
\ShowEq{polymap 42, y}
Согласно определению
\EqRef{norm of map, module}
\ShowEq{polymap 43, y}
Из неравенств
\EqRef{polymap 42, y},
\EqRef{polymap 43, y}
следует, что
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{polymap 4, x}
влечёт
\ShowEq{polymap 44, y}
Согласно определению
\ref{definition: continuous map, module},
отображение
$h$
непрерывно.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map is continuous, submaps}
\ShowEq{polymap 5, f}
тогда и только тогда, когда
\ShowEq{polymap 5, h}
\end{theorem}
\begin{remark}
Другими словами,
полилинейное отображение $f$ непрерывно тогда и только тогда, когда
отображение $h$ непрерывно и для любых
\ShowEq{polymap 5, a}
отображение
\ShowEq{polymap 3, algebra}
непрерывно.
\end{remark}
\begin{proof}
Утверждение, что из непрерывности отображения $f$ следует непрерывность
отображений $h$ и
\ShowEq{polymap 3, algebra},
следует из теорем
\ref{theorem: polylinear map f h()},
\ref{theorem: polylinear map f h}.

Пусть отображения $h$ и
\ShowEq{polymap 3, algebra}
непрерывны.
Согласно определению
\ref{definition: continuous multivariable map, module},
чтобы доказать непрерывность отображения $f$,
мы должны оценить разность
\ShowEq{polymap 5, y}
при условии
\DrawEq{|xi|<e, 1-n}{4}
Согласно равенству
\eqRef{f1n=hx}{convention},
\ShowEq{polymap 51, y}
Согласно равенству
\EqRef{polymap 51, y}
и утверждению
\ref{item: norm on D module 3, 2},
\ShowEq{polymap 52, y}
Согласно определению
\ref{definition: continuous map, module},
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta_1>0$, что
\ShowEq{|xn|<d1}
влечёт
\ShowEq{h(x)dx<e/2}
Рассмотрим второе слагаемое в правой части неравенства
\EqRef{polymap 52, y}.
\StartLabelItem{theorem: polylinear map is continuous, submaps}
\begin{enumerate}
\item Если $x_n=0$, то
\ShowEq{dh(x)x<e/2 1}
\label{item: dh(x)x<e/2 1}
\item  Поэтому мы положим $x_n\ne 0$.
Согласно определению
\ref{definition: continuous multivariable map, module},
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta_2>0$, что
\ShowEq{|xi|<d2}
влечёт
\ShowEq{dh(x)<e/2}
Из неравенств
\EqRef{dh(x)<e/2},
\EqRef{|fx|<|f||x|},
следует
\ShowEq{dh(x)x<e/2 2}
\label{item: dh(x)x<e/2 2}
\end{enumerate}
Следовательно, в обоих случаях
\RefItem{dh(x)x<e/2 1},
\RefItem{dh(x)x<e/2 2},
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta_2>0$, что
\ShowEq{|xi|<d2}
влечёт
\ShowEq{dh(x)x<e/2 3}
Пусть
\ShowEq{delta 1 2}
Из неравенств
\EqRef{polymap 52, y},
\EqRef{h(x)dx<e/2},
\EqRef{dh(x)x<e/2 3}
следует, что
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\DrawEq{|xi|<e, 1-n}{}
влечёт
\ShowEq{polymap 30, y}
Согласно определению
\ref{definition: continuous multivariable map, module},
отображение $f$ непрерывно.
\end{proof}

\begin{theorem}
\label{theorem: |f|=|h|}
Пусть
\ShowEq{Ai 1n}
- банахов $D$\Hyph модуль с нормой $\|x\|_i$.
Пусть $A$ - банахов $D$\Hyph модуль с нормой $\|x\|$.
Пусть
\ShowEq{f A1...An->A}
полилинейное отображение.
Пусть
\ShowEq{h 1n-1->A}
полилинейное отображение такое, что
\DrawEq{f1n=hx}{|f|=|h|}
Тогда
\ShowEq{|f|=|h|}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: norm of polylinear map}
\ShowEq{|hx1n-1|}
Согласно теореме
\ref{theorem: |fx|<|f||x|}
\ShowEq{|x|=|hx1n-1||xn|}
Из неравенств
\EqRef{|hx1n-1|},
\EqRef{|x|=|hx1n-1||xn|}
следует
\ShowEq{x h x1 xn}
Согласно теореме
\ref{theorem: |fx|<|f||x|1n}
\DrawEq{|fx|<|f||x|1n}{|f|=|h|}
Опираясь на теорему
\ref{theorem: |fx|<|f||x|1n}
и неравенства
\EqRef{x h x1 xn},
\eqRef{|fx|<|f||x|1n}{|f|=|h|},
мы имеем неравенство
\ShowEq{|f|<|h|}
Из равенства
\eqRef{f1n=hx}{|f|=|h|}
и неравенства
\eqRef{|fx|<|f||x|1n}{|f|=|h|}
следует, что
\ShowEq{|hx|/|xn|}
Из определения
\ref{definition: norm of polylinear map}
и неравенства
\EqRef{|hx|/|xn|}
следует, что
\ShowEq{|hx|<|f||x|}
Опираясь на теорему
\ref{theorem: |fx|<|f||x|1n}
и неравенства
\EqRef{|hx1n-1|},
\EqRef{|hx|<|f||x|},
мы имеем неравенство
\ShowEq{|h|<|f|}
Равенство
\EqRef{|f|=|h|}
следует из неравенств
\EqRef{|f|<|h|},
\EqRef{|h|<|f|}.
\end{proof}

\begin{theorem}
Полилинейное отображение $f$ непрерывно тогда и только тогда,
когда $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Мы докажем теорему индукцией по числу $n$ аргументов отображения $f$.
Для $n=1$, теорема является следствием теоремы
\ref{theorem: map is continuous iff}.

Пусть теорема верна для $n=k-1$.
Пусть
\ShowEq{A1k}
- банахов $D$\Hyph модуль с нормой $\|x\|_i$.
Пусть $A$ - банахов $D$\Hyph модуль с нормой $\|x\|$.
Мы можем представить полилинейное отображение
\ShowEq{f A1...Ak->A}
в следующем виде
\DrawEq{f1k=ha}{}
где
\ShowEq{h 1k-1->A}
полилинейное отображение.
Согласно теореме
\ref{theorem: polylinear map f h},
отображение $h$ является непрерывным полилинейным отображением $k-1$ переменной.
Согласно предположению индукции
\ShowEq{|h|<infty}
Согласно теореме
\ref{theorem: |f|=|h|},
\ShowEq{|f|=|h|<infty}
\end{proof}

\section{\texorpdfstring{$D$}{D}\hyph алгебра с базисом Шаудера}

\begin{definition}
\label{definition: Schauder basis}
Пусть $A$ - банахов $D$\Hyph модуль.\footnote{Определение
\ref{definition: Schauder basis}
дано на основе определения
\citeBib{4419-7514}-4.6, с. 182,
и леммы
\citeBib{4419-7514}-4.7, с. 183.}
Последовательность векторов
\ShowEq{Schauder basis}
называется
\AddIndex{базисом Шаудера}{Schauder basis},
если
\begin{itemize}
\item Множество векторов $e_{\gi i}$ линейно независимо.
\item Для каждого вектора $a\in A$ существует
единственная последовательность
\ShowEq{Schauder basis, coordinates}
такая, что
\DrawEq{Schauder basis, coordinates 0}{}
\end{itemize}
Последовательность
\ShowEq{ai in D}
называется
\AddIndex{координатами вектора
\ShowEq{a=ai ei}
относительно базиса Шаудера}
{coordinates of vector, Schauder basis}
$\Basis e$.
\qed
\end{definition}

Пусть $\Basis e$ - базис Шаудера банахова $D$\Hyph модуля $A$.
Мы будем говорить, что {\bf разложение}
\ShowEq{a=ae}
\AddIndex{вектора $a\in A$ относительно базиса $\Basis e$ сходится}
{expansion converges}.

\begin{theorem}
Пусть $\Basis e$ - базис Шаудера банахова $D$\Hyph модуля $A$.
Тогда
\ShowEq{Schauder basis, norm is finite, 1}
для любого вектора $a\in A$.
\end{theorem}
\begin{proof}
Из теоремы
\ref{theorem: normed module, norm of difference}
следует, что если
\ShowEq{Schauder basis, norm is finite, 2},
то мы не можем определить
\ShowEq{Schauder basis, norm is finite, 3}.
Следовательно, мы не можем разложить $a$ относительно базиса Шаудера.
\end{proof}

\begin{theorem}
\label{theorem: Schauder basis, limit}
Пусть $\Basis e$ - базис Шаудера банахова $D$\Hyph модуля $A$.
Пусть $a_i$ - координаты вектора $a$ относительно базиса $\Basis e$.
Тогда для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что
\ShowEq{Schauder basis, limit}
для любых $p$, $q>n_0$.
\end{theorem}
\begin{proof}
Неравенство
\EqRef{Schauder basis, limit, p}
является следствием определений
\ref{definition: limit of sequence, normed module},
\ref{definition: Schauder basis}.
Неравенство
\EqRef{Schauder basis, limit, p, q}
является следствием определений
\ref{definition: fundamental sequence, normed module},
\ref{definition: Schauder basis}.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{ai in I}
конечное семейство векторов банахова $D$\Hyph модуля $A$
с базисом Шаудера $\Basis e$.
Тогда\footnote{Смотри определение
\xRef{0701.238}{definition: linear span, vector space}
линейной оболочки в векторном пространстве.}
\ShowEq{span in A}
\end{theorem}
\begin{proof}
Для доказательства утверждения
\EqRef{span in A}
нам достаточно доказать следующие утверждения.
\begin{itemize}
\item
Если
\ShowEq{a1 a2 A}
то $a_1+a_2\in A$.

Так как 
\ShowEq{a1 a2 A}
то, согласно теореме
\ref{theorem: Schauder basis, limit},
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что
\ShowEq{Schauder basis, limit p12}
для любых $p$, $q>n_0$.
Из неравенств
\EqRef{Schauder basis, limit p12}
следует
\ShowEq{Schauder basis, limit p12 1}
Из неравенства
\EqRef{Schauder basis, limit p12 1}
следует, что последовательность
\ShowEq{Schauder basis, limit p12 2}
является фундаментальной.
\item
Если
\ShowEq{aA dD}
то $d\,a\in A$.

Так как 
\ShowEq{aA dD}
то, согласно теореме
\ref{theorem: Schauder basis, limit},
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что
\ShowEq{Schauder basis, limit p22}
для любых $p$, $q>n_0$.
Из неравенства
\EqRef{Schauder basis, limit p22}
следует
\ShowEq{Schauder basis, limit p22 1}
Из неравенства
\EqRef{Schauder basis, limit p22 1}
следует, что последовательность
\ShowEq{Schauder basis, limit p22 2}
является фундаментальной.
\end{itemize}
\end{proof}

\begin{theorem}
\label{theorem: Schauder basis, norm is finite}
Пусть $\Basis e$ - базис Шаудера банахова $D$\Hyph модуля $A$.
Тогда
\ShowEq{Schauder basis, norm is finite}
для любого вектора $e_{\gi i}$.
\end{theorem}
\begin{proof}
Пусть для
\ShowEq{Schauder basis, norm is finite, i=j}
Для любого
\ShowEq{Schauder basis, norm is finite, n>j}
если для последовательности
\ShowEq{ai in D}
верно, что
\ShowEq{Schauder basis, norm is finite, j}
Поэтому мы не можем сказать, определён ли вектор
\ShowEq{a=ai ei}
\end{proof}

Не нарушая общности, мы можем положить, что базис $\Basis e$
нормирован. Если предположить, что норма вектора
$e_{\gi i}$ отлична от $1$, то мы можем этот вектор
заменить вектором
\ShowEq{Banach algebra, normal basis, 1}
Согласно следствию
\ref{corollary: basis dual to normal basis is normal},
двойственный базис также является нормированным.

\begin{theorem}
\label{theorem: coordinates converges absolutely}
Пусть $\Basis e$ -
нормированый базис Шаудера банахова $D$\Hyph модуля $A$.
Пусть
\ShowEq{ai in D}
- такая последовательность, что
\ShowEq{ai in D 1}
Тогда существует предел\footnote{Смотри
аналогичные теоремы
\citeBib{Shilov single 3}, страница 60,
\citeBib{Fihtengolts: Calculus volume 2}, страницы 264, 295,
\citeBib{Smirnov vol 1}, страницы 293, 302.}
\DrawEq{Schauder basis, coordinates 0}{1}
\end{theorem}
\begin{proof}
Сущесвование предела
\eqRef{Schauder basis, coordinates 0}{1}
следует из неравенства
\ShowEq{Schauder basis, coordinates 2}
так как неравенство
\EqRef{Schauder basis, coordinates 2}
сохраняется при предельном переходе
\ShowEq{Schauder basis, coordinates 3}
\end{proof}

Пусть $\Basis e$ - нормированый базис Шаудера банахова $D$\Hyph модуля $A$.
Если
\ShowEq{ai in D 1}
то мы будем говорить, что {\bf разложение}
\ShowEq{a=ae}
\AddIndex{вектора $a\in A$ относительно базиса $\Basis e$
сходится нормально}
{expansion converges normally}.\footnote{Определение
нормальной сходимости разложения вектора относительно базиса
похоже на определение нормальной сходимости ряда.
Смотри \citeBib{Cartan differential form}, страница 12.}
Обозначим
\ShowEq{A plus Schauder}
множество векторов,
разложение которых относительно базиса $\Basis e$
сходится нормально.

\begin{theorem}
\label{theorem: |a|<|ai|}
Пусть $\Basis e$ - нормированый базис Шаудера банахова $D$\Hyph модуля $A$.
Если разложение
вектора $a\in A$ относительно базиса $\Basis e$
сходится нормально, то
\ShowEq{|a|<|ai|}
\end{theorem}
\begin{proof}
Из утверждения
\RefItem{norm on D module 3, 1}
следует, что
\ShowEq{|a|<|ai| 1}
Неравенство
\EqRef{|a|<|ai|}
следует из неравенства
\EqRef{|a|<|ai| 1}
и утверждения, что базис Шаудера $\Basis e$ является нормальным базисом.
\end{proof}

%\begin{convention}
%Пусть
%\ShowEq{f:A1->A2}
%отображение $D$\Hyph алгебры $A_1$ с базисом Шаудера $\Basis e_1$
%в $D$\Hyph алгебру $A_2$ с базисом Шаудера $\Basis e_2$.
%Мы будем требовать, что для любого вектора
%\ShowEq{e1 in}
%определён образ
%\ShowEq{f e1 in}
%при отображении $f$.
%\qed
%\end{convention}

\begin{theorem}
\label{theorem: linear map, module, Schauder basis}
Пусть
\ShowEq{f:A1->A2}
отображение $D$\Hyph модуля $A_1$ с базисом $\Basis e_1$ % Шаудера
в $D$\Hyph модуль $A_2$ с базисом Шаудера $\Basis e_2$.
Пусть $f^{\gi i}_{\gi j}$ - координаты отображения $f$
относительно базисов $\Basis e_1$ и $\Basis e_2$.
%Пусть
%\ShowEq{fij in D}
%для любого $\gi j$.
Тогда последовательность
\ShowEq{linear map, algebra, Schauder basis}
имеет предел для любого $\gi j$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из равенства
\ShowEq{f:A1->A2, 1}
%Утверждение теоремы следует из теоремы
%\ref{theorem: coordinates converges absolutely}.
\end{proof}

\begin{theorem}
\label{theorem: |fe|<|f|}
Пусть
\ShowEq{f:A1->A2}
отображение $D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
и нормированным базисом $\Basis e_1$ % Шаудера
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$
и базисом Шаудера $\Basis e_2$.
Тогда
\ShowEq{|fe|<|f|}
для любого $\gi i$.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: norm of map, module}
и определению
\ref{definition: normal basis},
неравенство
\EqRef{|fe|<|f|}
следует из неравенства
\ShowEq{|fe|<|f|, 1}
\end{proof}

\begin{remark}
\label{remark: module L(A1,A2) has Schauder basis}
Теорема
\ref{theorem: linear map, module, Schauder basis}
определяет ограничение на координаты отображения
$D$\Hyph модуля с базисом Шаудера.
Однако это ограничение можно сделать более строгим.
Пусть $A_1$ - $D$\Hyph модуль с нормированным базисом Шаудера $\Basis e_1$.
Пусть $A_2$ - $D$\Hyph модуль с нормированным базисом Шаудера $\Basis e_2$.
Согласно теореме
\ref{theorem: basis of module A1 A2},
$D$\Hyph модуль $\LDA$ имеет базис
\ShowEq{L(A1,A2) Schauder basis}
Поскольку базис $D$\Hyph модуля $\LDA$
является счётным базисом и $D$\Hyph модуль $\LDA$
имеет норму, мы требуем, чтобы рассматриваемый базис
был базисом Шаудера.
Согласно определению
\ref{definition: Schauder basis},
существует предел
\ShowEq{map in Schauder basis}
Из существования предела
\EqRef{map in Schauder basis}
следует существование предела последовательности
\EqRef{linear map, algebra, Schauder basis}.
Однако из существования предела
\EqRef{map in Schauder basis}
также следует что
\ShowEq{map in Schauder basis 1}
\qed
\end{remark}

\begin{theorem}
\label{theorem: |f|<epsilon}
Пусть
\ShowEq{f:A1->A2}
линейное отображение $D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
и нормированным базисом Шаудера $\Basis e_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$
и нормированным базисом Шаудера $\Basis e_2$.
Для любого
\ShowEq{epsilon in R}
существуют
$\gi N$, $\gi M$
такие, что
\DrawEq{|f|<epsilon}{theorem}
\end{theorem}
\begin{proof}
Согласно замечанию
\ref{remark: module L(A1,A2) has Schauder basis},
множество отображений
\ShowEq{basis of L(A1,A2)}
является базисом Шаудера $D$\Hyph модуля $\LDA$.
Следовательно, разложение
\ShowEq{fa=,5}
отображения $f$ сходится.
Согласно теореме
\ref{theorem: Schauder basis, limit},
для любого
\ShowEq{epsilon in R}
существуют
$\gi N$, $\gi M$
такие, что
\ShowEq{|f|<epsilon 1}
Согласно следствию
\ref{corollary: norm of basis L(A1,A2)},
неравенство
\eqRef{|f|<epsilon}{theorem}
следует из неравенства
\EqRef{|f|<epsilon 1}.
\end{proof}

\begin{theorem}
\label{theorem: |f|<F}
Пусть
\ShowEq{f:A1->A2}
линейное отображение $D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
и нормированным базисом Шаудера $\Basis e_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$
и нормированным базисом Шаудера $\Basis e_2$.
Существует
\ShowEq{F<infty}
такое, что
\ShowEq{|f|<<F}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: |f|<epsilon},
для заданого
\ShowEq{epsilon in R}
существуют
$\gi N$, $\gi M$
такие, что
\DrawEq{|f|<epsilon}{}
Так как $\gi N$, $\gi M$ конечны,
то существует
\ShowEq{F1=max f}
Мы получим неравенство
\EqRef{|f|<<F},
если положим
\ShowEq{F F1 epsilon}
\end{proof}

\begin{theorem}
\label{theorem: Schauder basis, image of map}
Пусть
\ShowEq{f:A1->A2}
линейное отображение $D$\Hyph модуля $A_1$ с нормой $\|x\|_1$
и нормированным базисом Шаудера $\Basis e_1$
в $D$\Hyph модуль $A_2$ с нормой $\|y\|_2$
и базисом Шаудера $\Basis e_2$.
Пусть
\ShowEq{|f|<infty}
Тогда для любого
\ShowEq{a1 in A1 plus}
образ
\DrawEq{f:A1->A2, 2}{Schauder}
определён корректно,
\ShowEq{a2 in A2 plus}
\end{theorem}
\begin{proof}
\ifx\texFuture\Defined
Пусть
\ShowEq{a1 in A1}
Согласно теореме
\ref{theorem: Schauder basis, limit},
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что
\ShowEq{a1 in A1, 1}
для любых $p$, $q>n_0$.
\fi
Из равенства
\EqRef{a1 in A1 plus}
и теоремы
\ref{theorem: |fe|<|f|}
следует
\ShowEq{|a2|<infty}
Из неравенства
\EqRef{|a2|<infty}
следует
\ShowEq{|a2|<infty 1}
Согласно теореме
\ref{theorem: coordinates converges absolutely},
образ $a_1\in A_1$ при отображении $f$ определён корректно.
\end{proof}

\begin{remark}
%\label{remark: }
Из доказательства теоремы
\ref{theorem: Schauder basis, image of map},
мы видим, что требование нормальной сходимости
разложения вектора относительно нормального базиса
является существенным.
Согласно замечанию
\ref{remark: module L(A1,A2) has Schauder basis},
если $A_i$, $i=1$, $2$,
- $D$\Hyph модуль с нормированным базисом Шаудера $\Basis e_i$,
то множество $\mathcal L(D;A_1;A_2)$ является
$D$\Hyph модулем с нормированным базисом Шаудера
\ShowEq{Basis e1 e2}.
Мы будем обозначать
\ShowEq{L plus A1 A2}
множество линейных отображений, разложение которых относительно базиса
\ShowEq{Basis e1 e2}
сходится нормально.
\qed
\end{remark}

\begin{theorem}
Пусть $A_1$
- $D$\Hyph модуль с нормой $\|x\|_1$
и нормированным базисом Шаудера $\Basis e_1$.
Пусть $A_2$
- $D$\Hyph модуль с нормой $\|x\|_2$
и нормированным базисом Шаудера $\Basis e_2$.
Пусть отображение
\ShowEq{f+A1->A2}
Тогда
\ShowEq{|f|<ij|f|}
\end{theorem}
\begin{proof}
Согласно следствию
\ref{corollary: norm of basis L(A1,A2)},
базис
\ShowEq{Basis e1 e2}
является нормированным базисом Шаудера.
Теорема следует из теоремы
\ref{theorem: |a|<|ai|}.
\end{proof}

\begin{corollary}
\label{corollary: |f|<infty}
Пусть $A_1$
- $D$\Hyph модуль с нормой $\|x\|_1$
и нормированным базисом Шаудера $\Basis e_1$.
Пусть $A_2$
- $D$\Hyph модуль с нормой $\|x\|_2$
и нормированным базисом Шаудера $\Basis e_2$.
Пусть отображение
\ShowEq{f+A1->A2}
Тогда
\ShowEq{|f|<infty}
\qed
\end{corollary}

\begin{theorem}
\label{theorem: s|ab|<s|a|s|b|}
Пусть
\ShowEq{a,b>0}
Тогда
\ShowEq{s|ab|<s|a|s|b|}
\end{theorem}
\begin{proof}
Докажем теорему индукцией по $n$.

Неравество
\EqRef{s|ab|<s|a|s|b|}
для $n=2$ является следствием неравенства
\ShowEq{s|ab|<s|a|s|b| n=2}

Пусть неравенство
\EqRef{s|ab|<s|a|s|b|}
верно для $n=k-1$.
Неравенство
\ShowEq{s|ab|<s|a|s|b| n=k}
является следствием неравенства
\EqRef{s|ab|<s|a|s|b| n=2}.
Из неравенства
\EqRef{s|ab|<s|a|s|b| n=k}
следует, что неравенство
\EqRef{s|ab|<s|a|s|b|}
верно для $n=k$.
\end{proof}

\begin{theorem}
\label{theorem: s|ab|<s|a|s|b| infty}
Пусть
\ShowEq{a,b>0 infty}
Тогда
\ShowEq{s|ab|<s|a|s|b| infty}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
ref{theorem: s|ab|<s|a|s|b|}
когда $n\rightarrow\infty$.
\end{proof}

\begin{theorem}
Пусть $A_i$, $i=1$, $2$, $3$,
- $D$\Hyph модуль с нормой $\|x\|_i$
и нормированным базисом Шаудера $\Basis e_i$.
Пусть отображение
\ShowEq{f+A1->A2}
Пусть отображение
\ShowEq{g+A2->A3}
Тогда отображение
\ShowEq{gf+A1->A3}
\end{theorem}
\begin{proof}
Согласно утверждению
\RefItem{norm on D module 3, 1}
\ShowEq{gf+A1->A3 1}
Из теоремы
\ref{theorem: s|ab|<s|a|s|b| infty}
и неравенства
\EqRef{gf+A1->A3 1}
следует, что
\ShowEq{gf+A1->A3 2}
Из неравенства
\EqRef{gf+A1->A3 2}
следует
\ShowEq{gf+A1->A3 3}
Теорема следует из неравенства
\EqRef{gf+A1->A3 3}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map, Schauder basis}
Пусть
\ShowEq{Ai 1n}
- $D$\Hyph модуль с нормой $\|x\|_i$
и нормированным базисом Шаудера $\Basis e_i$.
Пусть
$A$
- $D$\Hyph модуль с нормой $\|x\|$
и нормированным базисом Шаудера $\Basis e$.
Пусть
\ShowEq{A1...An->A}
полилинейное отображение,
\ShowEq{|f|<infty}
Пусть
\ShowEq{ai in Ai+}
Тогда
\ShowEq{a=f(a1...an) A+}
\end{theorem}
\begin{proof}
Мы докажем утверждение теоремы
индукцией по $n$.

Для $n=1$ утверждение теоремы следует из теоремы
\ref{theorem: Schauder basis, image of map}.

Пусть утверждение теоремы справедливо для $n=k-1$.
Пусть
\ShowEq{f A1...Ak-1 ->A}
полилинейное отображение,
\ShowEq{|f|<infty}
Мы можем представить отображение $f$ в виде композиции отображений
\DrawEq{f1k=ha}{}
Согласно теореме
\ref{theorem: |f|=|h|},
\ShowEq{|h|<infty}
Согласно предположению индукции
\ShowEq{h() in L+}
Согласно теореме
\ref{theorem: |fx|<|f||x|1n},
\ShowEq{|h()|<infty}
Согласно теореме
\ref{theorem: Schauder basis, image of map}
\ShowEq{h()a in A+}
\end{proof}

Согласно определению
\xRef{8433-5163}{definition: algebra over ring},
алгебра - это модуль, в котором произведение определено
как билинейное отображение
\ShowEq{xy=Cxy}
Мы будем требовать
\ShowEq{|C|<infty}

\begin{convention}
%\label{convention: }
Пусть $\Basis e$ - базис Шаудера свободной $D$\Hyph алгебры $A$.
Произведение базисных векторов в $D$\Hyph алгебре $A$
определено согласно правилу
\DrawEq{product of basis vectors}{Schauder basis}
где
\ShowEq{structural constants of algebra}
- \AddIndex{структурные константы}{structural constants}
$D$\Hyph алгебры $A$.
Так как произведение векторов базиса $\Basis e$
$D$\Hyph алгебры $A$ является вектором $D$\Hyph алгебры $A$, то
мы требуем, что
последовательность
\ShowEq{structural constants of algebra in Schauder basis}
имеет предел для любых $\gi i$, $\gi j$.
\qed
\end{convention}

\begin{theorem}
Пусть $\Basis e$ - базис Шаудера свободной $D$\Hyph алгебры $A$.
Тогда для любых
\ShowEq{a b in basis of algebra plus}
произведение, определённое согласно правилу
\DrawEq{product ab in algebra}{Schauder basis}
определено корректно.
При этом условии
\ShowEq{ab in A+}
\end{theorem}
\begin{proof}
Так как произведение в алгебре является билинейным отображением,
то произведение $a$ и $b$ можно записать в виде
\DrawEq{product ab in algebra, 1}{Schauder basis}
Из равенств
\eqRef{product of basis vectors}{Schauder basis},
\eqRef{product ab in algebra, 1}{Schauder basis},
следует
\DrawEq{product ab in algebra, 2}{Schauder basis}
Так как $\Basis e$ является базисом алгебры $A$, то равенство
\eqRef{product ab in algebra}{Schauder basis}
следует из равенства
\eqRef{product ab in algebra, 2}{Schauder basis}.

Из теоремы
\ref{theorem: polylinear map, Schauder basis}
следует, что
\ShowEq{ab in A+}
\end{proof}

\ifx\texFuture\Defined
\begin{theorem}
\label{theorem: standard component of tensor, algebra, Hamel basis}
Пусть $A_1$, ..., $A_n$ -
свободные алгебры над  коммутативным кольцом $D$.
Пусть $\Basis e_i$ - базис Гамеля $D$\Hyph алгебры $A_i$.
Тогда множество векторов
\ShowEq{tensor, algebra, Hamel basis}
является базисом Гамеля тензорного произведения
\ShowEq{tensor, algebra, Hamel basis, 1}
\end{theorem}
\begin{proof}
Для доказательства теоремы мы должны рассмотреть диаграмму
\xEqRef{8433-5163}{diagram top, algebra, tensor product},
которой мы пользовались для доказательства теоремы
\xRef{8433-5163}{theorem: tensor product of algebras is module}
\ShowEq{standard component of tensor, algebra, Hamel basis, diagram}
Пусть $M_1$ - модуль над кольцом $D$, порождённый
произведением $\Times$
$D$\Hyph алгебр $A_1$, ..., $A_n$.
\begin{itemize}
\item
Пусть вектор $b\in M_1$ имеет конечное разложение
относительно базиса $\Times$
\ShowEq{b in M_1, Hamel basis}
где $I_1$ - конечное множество.
Пусть вектор $c\in M_1$ имеет конечное разложение
относительно базиса $\Times$
\ShowEq{c in M_1, Hamel basis}
где $I_2$ - конечное множество.
Множество
\ShowEq{I=I1+I2}
является конечным множеством.
Положим
\ShowEq{b I2, c I1}
Тогда
\ShowEq{b+c in M_1, Hamel basis}
где $I$ - конечное множество.
Аналогично, для $d\in D$
\ShowEq{db in M_1, Hamel basis}
где $I_1$ - конечное множество.
Следовательно, мы доказали следующее утверждение.\footnote{Множество
$\Times$ не может быть базисом Гамеля, так как
это множество не счётно.}
\begin{lemma}
\label{lemma: M is submodule}
Множество $M$ векторов модуля $M_1$, имеющих конечное разложение
относительно базиса $\Times$, является подмодулем модуля $M_1$.
\end{lemma}
\end{itemize}
Инъекция
\ShowEq{map i, algebra, tensor product, 1}
определена по правилу
\ShowEq{map i, algebra, Hamel basis, tensor product}
Пусть $N\subset M$ - подмодуль, порождённый элементами вида
\ShowEq{kernel, algebra, Hamel basis, tensor product}
где $d_i\in A_i$, $c_i\in A_i$, $a\in D$.
Пусть
\[
j:M\rightarrow M/N
\]
каноническое отображение на фактормодуль.
Поскольку элементы \EqRef{kernel 1, algebra, Hamel basis, tensor product}
и \EqRef{kernel 2, algebra, Hamel basis, tensor product}
принадлежат ядру линейного отображения $j$,
то из равенства
\EqRef{map i, algebra, Hamel basis, tensor product}
следует
\ShowEq{f, algebra, Hamel basis, tensor product}
Из равенств \EqRef{f 1, algebra, Hamel basis, tensor product}
и \EqRef{f 2, algebra, Hamel basis, tensor product}
следует, что отображение $f$ полилинейно над кольцом $D$.

Модуль $M/N$ является тензорным произведением $A_1\otimes...\otimes A_n$,
отображение $j$ имеет вид
\ShowEq{map j, Hamel basis}
и множество
тензоров вида
\ShowEq{tensor, algebra, Hamel basis}
является счётным базисом модуля $M/N$.
Согласно лемме
\ref{lemma: M is submodule},
произвольный вектор
\ShowEq{b in M, Hamel basis, 0}
имеет представление
\ShowEq{b in M, Hamel basis}
где $I$ - конечное множество.
Согласно определению
\EqRef{map j, Hamel basis}
отображения $j$
\ShowEq{j(b), Hamel basis}
где $I$ - конечное множество.
Так как $\Basis e_k$ - базис Гамеля $D$\Hyph алгебры $A_k$,
то для любого набора индексов $k\cdot i$, в равенстве
\ShowEq{aki, Hamel basis}
множество значений
\ShowEq{aki 1, Hamel basis}
отличных от $0$, конечно.
Следовательно, равенство
\EqRef{j(b), Hamel basis}
имеет вид
\ShowEq{j(b), 1, Hamel basis}
где множество значений
\ShowEq{j(b), 2, Hamel basis}
отличных от $0$, конечно.
\end{proof}

\begin{corollary}
\label{corollary: tensor product, Hamel basis}
Пусть $A_1$, ..., $A_n$ -
свободные алгебры над  коммутативным кольцом $D$.
Пусть $\Basis e_i$ - базис Гамеля $D$\Hyph алгебры $A_i$.
Тогда произвольный тензор $a\in A_1\otimes...\otimes A_n$
имеет конечное множество стандартных компонент,
отличных от $0$.
\qed
\end{corollary}

\begin{theorem}
Пусть $A_1$ - алгебра
над кольцом $D$.
Пусть $A_2$ - свободная ассоциативная алгебра
над кольцом $D$ с базисом Гамеля $\Basis e$.
Отображение
\ShowEq{standard representation of map A1 A2, 1, Hamel basis}
порождённое отображением $f\in\LDA$
посредством тензора $a\in\ATwo$, имеет стандартное представление
\ShowEq{standard representation of map A1 A2, 2, Hamel basis}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: standard component of tensor, algebra, Hamel basis},
стандартное представление тензора $a$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, Hamel basis}
Равенство
\EqRef{standard representation of map A1 A2, 2, Hamel basis}
следует из равенств
\EqRef{standard representation of map A1 A2, 1, Hamel basis},
\EqRef{standard representation of map A1 A2, 3, Hamel basis}.
\end{proof}
\fi



==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%A%0
\Symb%
   {минорная матрица}%
   {A from b a}%
\Symb%
   {минорная матрица}%
   {A from columns T}%
\Symb%
   {минорная матрица}%
   {A from rows S}%
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
\Symb%
   {минорная матрица}%
   {A without column a}%
\Symb%
   {минорная матрица}%
   {A without columns T}%
\Symb%
   {минорная матрица}%
   {A without row b}%
\Symb%
   {минорная матрица}%
   {A without rows S}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 1}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 2}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
\Symb%
   {аффинное пространство}%
   {affine space, division ring}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения $A$ $D$\Hyph векторного пространства}%
   {component of linear map, D vector space}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {CR linear combination in A module}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {левая дробь}%
   {left fraction}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
\Symb%
   {главный идеал}%
   {principal ideal}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Symb%
   {правый сдвиг}%
   {starT shift}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {левый сдвиг}%
   {Tstar shift}%
\Symb%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {правая дробь}%
   {right fraction}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
\Symb%
   {тензорное произведение представлений}%
   {tensor product of representations}%

\SetIndexSpace%C%0
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
\Symb%
   {структурные константы}%
   {structural constants}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {координаты базового вектора представления группы Ли}%
   {basis vector of representation of Lie group, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, scalar}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
\Symb%
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 1, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 2, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 3, D vector space}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 1, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 2, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 3, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Symb%
   {\drc векторное пространство \subs строк}%
   {r rows drc vector space}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Symb%
   {тензорная степень тела $D$}%
   {tensor power of division ring}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Symb%
   {матрица Якоби левого сдвига}%
   {aE, quaternion, Jacobian matrix}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
\Symb%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 1}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 2}%
\Symb%
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {координаты базиса в \rcd векторном пространстве \sups строк}%
   {basis coordinates, c rows rcd vector space}%
\Symb%
   {координаты базиса в \drc векторном пространстве \subs строк}%
   {basis coordinates, r rows drc vector space}%
\Symb%
   {базис в \rcd векторного пространства \sups строк}%
   {basis, c rows rcd vector space}%
\Symb%
   {базис в \drc векторном пространстве \subs строк}%
   {basis, r rows drc vector space}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма функционала}%
   {norm of functional}%
\Symb%
   {норма отображения}%
   {norm of map}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of Tstar representation of group}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Symb%
   {сумма линейных отображений}%
   {sum of linear maps}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {алгебра Ли группы Ли}%
   {g}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator I of representation}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
\Symb%
   {вектор отображения $f$}%
   {vector of mapping}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%

\SetIndexSpace%L%0
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {множество \Acr линейных отображений модуля $\Vector V$ в модуль $\Vector W$}%
   {set Acr linear maps, module}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
\Symb%
   {\rcd векторное пространство линейных отображений \drc векторного пространства $ V$ в \drc векторное пространство $W$}%
   {set linear maps, drc vector space}%
\Symb%
   {\drc векторное пространство линейных отображений \rcd векторного пространства $V$ в \rcd векторное пространство $W$}%
   {set linear maps, rcd vector space}%
\Symb%
   {множество линейных отображений}%
   {set linear maps, scalar}%
\Symb%
   {множество линейных отображений}%
   {set linear maps, vector}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {множество \Ts преобразований универсальной алгебры $M$}%
   {set of Tstar transformations}%
\Symb%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {\rcd векторное пространство \sups строк}%
   {c rows rcd vector space}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
\Symb%
   {скаляр отображения $f$}%
   {scalar of mapping}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%
\Symb%
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%

\SetIndexSpace%T%0
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Symb%
   {касательная плоскость к группе $G$}%
   {TaG}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%

\SetIndexSpace%V%0
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

